SAS-Assisted Coexistence-Aware Dynamic Channel Assignment in CBRS Band

The paradigm of shared spectrum allows secondary devices to opportunistically access spectrum bands underutilized by primary owners. Recently, the FCC has targeted the sharing of the 3.5 GHz (3550-3700 MHz) federal spectrum with commercial systems such as small cells. The rules require a Spectrum Access System (SAS) to accommodate three service tiers: 1) Incumbent Access, 2) Priority Access (PA), and 3) Generalized Authorized Access (GAA). In this work, we study the SAS-assisted dynamic channel assignment (CA) for PA and GAA tiers.We introduce the node-channel-pair conflict graph to capture pairwise interference, channel and geographic contiguity constraints, spatially varying channel availability, and coexistence awareness. The proposed conflict graph allows us to formulate PA CA and GAA CA with binary conflicts as max-cardinality and max-reward CA, respectively. Approximate solutions can be found by a heuristic-based algorithm that search for the maximum weighted independent set. We further formulate GAA CA with non-binary conflicts as max-utility CA. We show that the utility function is submodular, and the problem is an instance of matroid-constrained submodular maximization. A polynomial-time algorithm based on local search is proposed that provides a provable performance guarantee. Extensive simulations using a real-world Wi-Fi hotspot location dataset are conducted to evaluate the proposed algorithms. Our results have demonstrated the advantages of the proposed graph representation and improved performance of the proposed algorithms over the baseline algorithms.

==> ArXiv Submission/sections/abstract.tex <==
\begin{abstract}
The paradigm of shared spectrum allows secondary devices to opportunistically access spectrum bands underutilized by primary owners. 
\rev{Recently}, the FCC \rev{has} targeted \rev{the} sharing \rev{of} the 3.5 GHz (3550-3700 MHz) federal spectrum with commercial systems such as small cells. 
The %proposed 
rules require a Spectrum Access System (SAS) to \rev{accommodate three service tiers: 1) Incumbent Access,} 2) Priority Access (PA), and 3) Generalized Authorized Access (GAA).
In this work, we study the SAS-assisted dynamic channel assignment (CA) for \rev{PA and GAA tiers}. 
We introduce the node-channel-pair conflict graph to capture pairwise interference, channel and geographic contiguity constraints, spatially varying channel availability, and coexistence \rev{awareness}. 
%A super-node formation algorithm is developed to identify valid super-nodes, i.e., a set of nodes that can coexist on the same channel(s) via time-division-multiplexing-based MAC protocols. 
\rev{The proposed graph representation allows us to} formulate PA CA and GAA CA with binary conflicts as max-cardinality and max-reward CA, respectively.
\rev{Approximate solutions can be found by a heuristic-based algorithm that searches for the maximum weighted independent set.}
\rev{We further formulate GAA CA with non-binary conflicts  as max-utility CA.}
\rev{We show} that the utility function is submodular, and the problem is an instance of matroid-constrained submodular maximization. 
A local-search-based polynomial-time algorithm is proposed that provides a provable performance guarantee.
\rev{Extensive simulations using a real-world Wi-Fi hotspot location dataset are performed} to evaluate the proposed algorithms.
Our results have demonstrated the advantages of the proposed graph representation and improved performance of the proposed algorithms over the baseline algorithms.

\end{abstract}

\begin{IEEEkeywords}
\rev{Citizens Broadband Radio Service, 3.5 GHz Band}, Channel Assignment, Node-Channel Pair Conflict Graph, Coexistence Awareness, Maximum Weighted Independent Set, Submodular Maximization
\end{IEEEkeywords}

==> ArXiv Submission/sections/channel_assignment_binary.tex <==
\section{Novel Conflict Graphs and Problem Formulation}\label{sec:conflict_graph}
%As discussed in Section~\ref{sec:channel_assignment_scenario}, there exist a lot of dependencies among individual channel assignments in PA-CA and GAA-CA.
%In order to capture such dependencies, one way is the conflict graph representation \cite{?}, in which each vertex is typically a node (i.e., service area or CBSD in our case), and each edge indicates a conflict due to (co-channel) interference between the connected nodes. 
%Variants of conflict graphs are able to capture ... \cite{?}. 
%Unfortunately, node-based conflict graph cannot capture channel availability and contiguity conveniently. 

\rev{In order to incorporate channel availability and contiguity}, we define a NC pair as a channel assignment that assigns a set of contiguous and available channels to a node, i.e., a PA service area or a GAA node.
We then \rev{introduce} the NC-pair conflict graph, where each vertex is a NC pair and each edge indicates a conflict. %between two connected NC pairs due to the one-channel-assignment-per-node or interference constraint. 
In \rev{the rest of this section}, we will describe conflict graph construction in detail and present our problem formulation for each CA scenario.

\subsection{Conflict Graph for PA CA}
\rev{Let us} consider a geographic region with $M$ PA licensees. 
Each licensee $i$ holds $N_i$ PALs in $n_i$ service areas,
%Each service area consists of \rev{one or more} contiguous license areas with the same number of PALs. 
and there are a total of $n=\sum_{i=1}^M n_i$ service areas in total. 
%Although not explicitly required, it makes more sense to impose the second constraint, which also facilitates channel assignment.
%As a result, a license area may belong to different service areas for the same operator (see Fig.~\ref{fig:service_area_ex}), and channel contiguity is enforced in each service area. 
%\begin{figure}[ht!]
%   \centering
%   \includegraphics[width=0.6\columnwidth]{./figs/service_area_ex}
%   \caption{Example of defining service areas for an operator with three and two PALs in tracts 1 and 2, respectively. 
%    }
%    \label{fig:service_area_ex}
%\end{figure}
Let $S_{ij}$ be the set of license areas that form the $j$-th service area of licensee $i$, and each license area in $S_{ij}$ has $N_{ij}$ PALs\footnote{The constraint that no more than seven PALs shall be assigned in any license area should have been enforced during the licensing stage and can be verified by checking $\sum_{i=1}^M \sum_{j=1}^{n_i} \bold{1}_{\{s \in S_{ij}\}} \cdot N_{ij} \leq 7$ for each license area $s$, where $\bold{1}_{\{s \in S_{ij}\}}$ is the indicator variable.}.
There are a total of $10$ PAL channels in the CBRS, denoted as $\Omega=\{1,2,...,10\}$.
Due to the \rev{DPAs} of incumbents, the set of available PAL channels for $S_{ij}$, denoted as $\Gamma(S_{ij})$, is a subset of $\Omega$. 
%Since $N_{ij}$ contiguous channels need to be assigned to $S_{ij}$, the set of valid channel assignments $\mathcal{C}_{ij}$ is limited.
Denote the set of valid channel assignments for $S_{ij}$ as $\mathcal{C}_{ij}$. 
It means that each channel assignment $C \in \mathcal{C}_{ij}$ consists of contiguous channels and satisfies the conditions $C\in \Gamma({S_{ij}})$ and $|C| = N_{ij}$. 
For instance, with $\Gamma(S_{ij})=\{1,2,3\}$ and $N_{ij}=2$, we have $\mathcal{C}_{ij}=\{ \{1,2\}, \{2,3\}\}$.

In the proposed conflict graph $G=(V,E)$ for PA CA, each vertex is a NC pair $(S_{ij}, C_{ij})$ that assigns channel(s) $C_{ij}$ to $S_{ij}$, and an edge exists between $(S_{ij}, C_{ij})$ and $(S_{lk}, C_{lk})$, if
\begin{itemize}
\item $i=j$ and $l=k$ (i.e., $S_{ij}$ and $S_{lk}$ refer to the same service area), and $C_{ij} \neq C_{lk}$, or

%\item adjacent-node-geographic-contiguity constraint: for vertices $v,u\in V$, $S(v)$ and $S(u)$ are adjacent and belong to the same user, but 

\item $S_{ij}\cap S_{lk} \neq \emptyset$ and $C_{ij} \cap C_{lk} \neq \emptyset$.

\end{itemize} 
The first constraint requires each service area to take at most one channel assignment, referred to as the \textit{one-channel-assignment-per-node constraint}, while
the second constraint prevents two overlapping service areas from being assigned overlapping channels, which is called the \textit{conflict constraint}. 
\res{It is worth noting that by selecting a vertex $(S_{ij}, C_{ij})$, that is, assigning channel(s) $C_{ij}$ to $S_{ij}$, the SAS can meet both the geographic and channel contiguity requirements.}
An example of the proposed conflict graph for PA CA is provided in Fig.~\ref{fig:PA_conflict_graph_ex}.

\begin{figure}[ht!]
	\centering
	%	%\includegraphics[width=0.5\columnwidth]{./figs/PA_conflict_graph_ex}
	\includegraphics[width=0.6\columnwidth]{./figs/PA_conflict_graph_ex}
	\caption{
		Conflict graph for the PA CA example in Fig.~\ref{fig:channel_assignment_example}. 
		Dashed and solid edges are due to the one-channel-assignment-per-node and conflict constraints, respectively. 
		The SAS aims to choose the largest set of conflict-free vertices. 
		One possible CA scheme consists of two vertices in red, i.e, $(S_A, \{1\})$ and $(S_B, \{2,3\})$. 
		An alternative is $(S_A, \{3\})$ and $(S_B, \{1,2\})$.
	}
	\label{fig:PA_conflict_graph_ex}
\end{figure}

\res{Since a conflict due to interference exists only for two NC pairs that represent two overlapping service areas with overlapping channels, a sparse conflict graph would be expected in practice.
Therefore, adjacency lists would be preferred in general with a storage cost of $O(|V|+|E|)$. It takes $O(1)$ time to add a vertex or edge, $O(E)$ to remove a vertex, and $O(V)$ to remove an edge.
More details are available in \cite{cormen2009introduction}.}

%Now let us again consider the example in Fig.~\ref{fig:channel_assignment_example}.
%In addition, we assume that B also holds 2 PALs in tract 2.
%Hence, A's service area is $S_A = \{\text{Tract }1, \text{Tract }2\}$ with one PAL, and B's service area is $S_B = \{\text{Tract }2, \text{Tract }3\}$ with two PALs. 
%The corresponding conflict graph is shown in Fig.~\ref{fig:PA_conflict_graph_ex}. 
%


\noindent \textbf{Problem Formulation:}
Given a conflict graph $G(V,E)$ for PA CA, the SAS wants to find a scheme $I \subseteq V$ so as to maximize the total number of served service areas without conflicts,
\begin{align}
\max_{I \subseteq V} &~|I| \nonumber \\
\text{Subject to: } e(u, v) & \notin E, \forall u,v\in I,\label{eq:max_cardinality_CA}
\end{align}
%\begin{align}
%\max_{I \subseteq V} |I|\text{, s.t. } e(u, v) & \notin E, \forall u,v\in I,\label{eq:max_cardinality_CA}
%\end{align}
where $|\cdot|$ is the cardinality operator.
%This problem is the classic \textit{Maximum Independent Set (MIS)} problem in graph theory \cite{?}. 
We refer to the above problem as \textbf{Max-Cardinality CA}. 
%\footnote{Due to the one-channel-assignment-per-node constraint, the maximum possible size of $I$ is $n$. In practice, the PAL licensing process should ensure that a solution of size $n$ can be found. When it is impossible to do so due to incumbent activities, the SAS may have to temporarily divide a large service areas to smaller ones that take non-contiguous channels. }.



%Alternatively, PA-CA may be formulated as a Integer Linear Programming (ILP) problem: let $I_i$ be the indicator variable for the $i$-th vertex, which is $1$ when selected and $0$ otherwise. The SAS wants to find a scheme $\{I_i:I_i \in \{0,1\}\}$ so as to 
%\begin{align*}
%\max \sum_{i=1}^{|V|} I_i, \text{ s.t. }  \sum_{j=1}^{|V|} e_{ij} I_j \leq 1, \forall i=1,2,...,|V|,
%\end{align*}
%where $e_{ij}=1$ means that the $i$-th and $j$-th vertices conflict with each other, and $e_{ij}=0$ otherwise.


%\begin{figure*}[t]
%    \centering
%    \begin{subfigure}[b]{.30\textwidth}
%    		\centering
%        \includegraphics[width=1\textwidth]{./figs/protocol_model_case1}
%        \caption{No conflict.}
%        \label{fig:protocol_model_case1}
%    \end{subfigure}
%    ~ 
%    \begin{subfigure}[b]{.30\textwidth}
%    		\centering
%        \includegraphics[width=.8\textwidth]{./figs/protocol_model_case2}
%        \caption{Type-I conflict.}
%        \label{fig:protocol_model_case2}
%    \end{subfigure}
%    ~
%    \begin{subfigure}[b]{.30\textwidth}
%    		\centering
%        \includegraphics[width=.6\textwidth]{./figs/protocol_model_case3}
%        \caption{Type-II conflict.}
%        \label{fig:protocol_model_case3}
%    \end{subfigure}
%    \caption{Impact of CBSD $j$'s interference on CBSD $i$. 
%    }
%    \label{fig:protocol_model}
%\end{figure*}

\subsection{Conflict Graph with Binary Conflicts for GAA CA }
\label{sec:conflict_graph_binary}
Suppose that there are $n$ GAA nodes at fixed locations in the same geographic region. 
The ground set of channels is $\Omega = \{1,2,...,15\}$, and the SAS can determine the set of available channels $\Gamma(i) \subseteq \Omega$ %based on 1) PPAs and \rev{PA channel assignments,} 2) registration information including location and installation/operating parameters, and 3) \rev{the physical interference model} and interference requirements. 
for each GAA node $i$. 
In this paper, we focus on CA by assuming fixed transmit power for all nodes and leave joint channel and power assignment as future work.

Denote \rev{the demand set of} node $i$ as $\mathcal{D}(i)=\{d_{i1}, d_{i2},...\}$, where $d_{ik}$ is the number of contiguous channels \rev{node $i$ requests}. 
For example, $\mathcal{D}(i)=\{2,4\}$ means that node $i$ requests for two or four contiguous channels.
By default, the SAS may set $\mathcal{D}(i)$ to $\{1,2,...,L\}$, where $L$ is the limit (e.g., $L=4$). 
As a result, $\Gamma(i)$ and $\mathcal{D}(i)$ jointly determine the set of valid channel assignments $\mathcal{C}(i)$.
For example, with $\Gamma(i)=\{1,4,5\}$ and $\mathcal{D}(i)=\{1,2\}$, we have $\mathcal{C}(i) = \{\{1\}, \{4\}, \{5\}, \{4,5\}\}$. 

%It is easy to see that channel availability and flexible demands with contiguity have been accounted for when the SAS determines $\mathcal{C}(i)$. 

In the proposed conflict graph $G(V,E)$ for \rev{binary} GAA CA, each vertex is a NC pair $(i, C_i)$ that assigns channel(s) $C_i \in \mathcal{C}(i)$ to node $i$, and an edge exists between $(i,C_i)$ and $(j,C_j)$ if 
\begin{itemize}
\item $i=j$ and $C_i \neq C_j$, or 

\item $i\neq j$, $C_i \cap C_j \neq \emptyset$, and node $i$ would conflict or interfere with node $j$ when assigned the same channel based on the interference model.
%, according to the interference model described below. 
\end{itemize}
\rev{The above two conditions correspond to the one-channel-assignment-per-node constraint and the conflict/interference constraint, respectively.}
%the first constraint is the  one-channel-assignment-per-node constraint, and the second constraint is the conflict or interference constraint. 
\res{Like the conflict graph for PA CA, the conflict graph for GAA CA is expected to be sparse and thus adjacency lists are generally preferred.}

In the rest of this section, we will characterize pairwise interference relationship, discuss coexistence awareness under binary conflicts, and introduce a reward function to reflect preferences of NC pairs. 
Then we will present our problem formulation for binary GAA CA.

%Next, we will present our interference model in more details. 


%It is important to note that the size of $V$ in the proposed conflict graph expands as compared to node-based conflict graphs \rev{[cite]}, it still increases linearly in $n$ thanks to channel contiguity.
%To see why, consider the worst case where all channels in $\Omega$ are available, and each node requests any number of channels between $1$ and $L$.
%Then the number of NC pairs for each node is at most $L|\Omega|$, which is a constant, and thus the size of $V$ is at most $L|\Omega|n$ or $\mathcal{O}(n)$.

%Next we will discuss our interference model in more details. 


\begin{figure*}[!t]
	\centering
	\subfloat[]{\includegraphics[width=.3\textwidth]{./figs/protocol_model_case1}
		\label{fig:protocol_model_case1}}
	%\hfil
	~
	\subfloat[]{\includegraphics[width=.24\textwidth]{./figs/protocol_model_case2}
		\label{fig:protocol_model_case2}}
	~~~~~~
	\subfloat[]{\includegraphics[width=.18\textwidth]{./figs/protocol_model_case3}
		\label{fig:protocol_model_case3}}
	\caption{Impact of node $j$'s interference on node $i$. 
		(a) No conflict. Nodes $i$ and $j$ are free to reuse the same channel if $j$'s interference region does not overlap with $i$'s service region. 
		(b) Type-I conflict. Node $j$ causes non-negligible interference to $i$'s clients located in the overlapping region, which cannot be detected by $i$ \rev{without feedback from the clients such as packet loss or throughput degradation}. 
		(c) Type-II conflict. Node $j$ is within $i$'s CS or ED range, and its interference can detected by $i$.
	}
	\label{fig:protocol_model}
	
\end{figure*}

\subsubsection{Characterization of Pairwise Interference}\label{sec:interference_model}
First of all, the SAS needs to determine whether two GAA nodes are interfering with each other, which is a binary (yes-or-no) decision. 
%\revv{According to the physical interference model \cite{gupta2000capacity}, a successful reception at a client from the $i$-th CBSD is possible, if the SINR at the client is greater than a certain threshold $SINR_{\min}$. If client locations are known, the SAS can use this criterion to determine the pairwise interference relationship. Otherwise, the SAS may consider the worst-case scenario where clients are located at the service region boundaries with respect to a certain signal level (denoted as $\gamma_i$) and determine if the interference from node $j$ (denoted as $\gamma_{i,j}$) at the nearest boundary client exceeds $SINR_{\min}$, i.e., $\frac{\gamma_i}{ \sigma_n^2 + \gamma_{i,j}}\geq SINR_{\min}$, where $\sigma_n^2$ is the noise power. This determines the maximum allowable interference from node $j$ on node $i$, that is, $\gamma_{i,j} \leq \gamma_i/SINR_{\min}-\sigma_n^2$. In this work, we assume that the SAS has no prior knowledge about client locations\footnote{Clients or end user devices are not required to register with the SAS or report their locations.}, and thus determining the pairwise interference relationship translates into determining whether node $i$'s service region overlaps with node $j$'s interference region. Nevertheless, the client location information, if available, can be exploited to determine the interference relationship more accurately.}
%\revv{While the service and interference regions can be highly irregular in practice, we assume circular regions for illustration.}
Similar to the interference protection for PA users, the SAS may decide that node $j$ is interfering with $i$, if the received interference from node $j$ at any location within $i$'s service contour (e.g., the $-96$ dBm/$10$ MHz contour) exceeds a certain limit (e.g., $-80$ dBm/$10$ dBm).
%\cite{gupta2000capacity,mishra2006client, niculescu2007interference}
Denote node $i$'s service region as $\mathcal{R}_i$ of radius $r_i$ and node $j$'s interference region as $\mathcal{R}_{j,int}$ of radius $r_{j, int}$.
Then there exists no conflict between $i$ and $j$ \rev{due to $j$' interference}, if the distance is larger than $r_i + r_{j,int}$, regardless of the positions of $i$'s clients (Fig.~\ref{fig:protocol_model_case1}).

As nodes $i$ and $j$ get closer,  $\mathcal{R}_{j,int}$ starts to overlap with $\mathcal{R}_{i}$, which means that $j$ may cause interference to clients that are possibly located in the overlapping region in the downlink. 
If the distance is smaller than $r_i + r_{j,int}$ but larger than $i$'s CS/ED range $r_{i,cs}$, as shown in Fig.~\ref{fig:protocol_model_case2}, node $j$ is said to be hidden from $i$, and the interference from $j$ cannot be detected by $i$ \rev{without feedback from $i$'s clients}.
When the distance is less than $r_{i,cs}$ (Fig.~\ref{fig:protocol_model_case3}), node $i$ is able to detect $j$'s transmission via CS/ED and 
%back off \rev{following the Wi-Fi like} MAC protocols to 
%mitigate the adverse impact of interference and 
achieve %harmonious 
co-channel coexistence \rev{through contention}. 
In order to distinguish the above cases, we call them type-I and type-II conflicts, respectively. 
\rev{Note that} our interference model is very similar to the popular protocol models in literature (e.g., \cite{gupta2000capacity,mishra2006client, niculescu2007interference}), \rev{which} can be easily implemented in the SAS using radio propagation models.
%Moreover, if client information and feedback (e.g., location and measurement reports) is available, the SAS can exploit it to determine the pairwise interference relationship between two nodes more accurately \rev{[cite]} \cite{mishra2006client}.


\subsubsection{Coexistence Awareness}\label{sec:coexistence_awareness}
Ideally, two nodes should be assigned the same channel only when they do not conflict.
Nevertheless, \rev{GAA nodes have the lowest spectrum access priority} and are expected to coexist in the presence of conflicts.
Compared with type-I conflicts, type-II conflicts can be  handled more easily and thus may be considered as coexistence opportunities to the SAS.  
To that end, we introduce \textit{super-NC pair} $(S,C)$, where $S$ is \rev{a \textit{super-node}} that consists of nodes that can coexist on channel $C$ \rev{with two conditions: 1) channel $C$ is available at all nodes in $S$ and 2)} nodes in $S$ be within each other's CS/ED range so that all conflicts can be gracefully resolved.
The super-node formation algorithm will be presented later in Section~\ref{sec:super_node_formation}.

Fig.~\ref{fig:GAA_conflict_graph_ex} shows an example of the proposed conflict graph \rev{with and without coexistence awareness}.
\rev{Suppose that} nodes B, C are within each other's CS/ED range. \rev{Then} there are two super-NC pairs $(\{B,C\}, \{1\})$ and $(\{B,C\}, \{2\})$.
\rev{As illustrated in Fig.~\ref{fig:GAA_interference_graph_with_coex}}, 
when a super-NC pair is identified, it is added to the graph and inherits the conflict relationship of its children RC pairs. 
Then edges among its children RC pairs are removed.  
For instance, removing the edge between $(B,\{2\})$ and $(C,\{2\})$ means that \rev{when} $(B,\{2\})$ is selected, $(\{B,C\},\{2\})$ \rev{will become} invalid, but the SAS can still select $(C,\{2\})$, \rev{since B and C are able to resolve type-II conflicts. } 

\begin{figure}[!t]
	\centering
	\subfloat[]{\includegraphics[trim=0 0.8cm 0 0.8cm,clip=true,width=.7\columnwidth]{./figs/GAA_conflict_graph_no_coex}
		\label{fig:GAA_interference_graph_no_coex}}
	
	\subfloat[]{\includegraphics[width=.7\columnwidth]{./figs/GAA_conflict_graph_with_coex}
		\label{fig:GAA_interference_graph_with_coex}}
	\caption{
		Example of (a) NC-pair conflict graph and (b) coexistence-aware NC-pair conflict graph.
		Suppose that A has two channels $\{2,3\}$ available and requests for two contiguous channel, while B and C have two available channels $\{1,2\}$ and each requests for one channel. 
		A, B, and C are interfering with each other, but B and C are within each other's CS/ED range. 
		Based on the \rev{conflict graph} in (a), the SAS may assign CH $\{2,3\}$ to A and CH $\{1\}$ to C. 
		Realizing that B and C are able to \rev{coexist under type-II conflicts, }%detect each other's interference and coexist harmoniously, 
		the SAS may assign CH $\{1\}$ to both B and C based on the conflict graph in (b). 
	}
	\label{fig:GAA_conflict_graph_ex}
\end{figure}


%\begin{figure}[!ht]
%	\centering
%	\subfloat[]{\includegraphics[width=.25\columnwidth]{./figs/GAA_interference_graph_ex}
%		\label{fig:GAA_interference_graph_ex}}
%	\subfloat[]{\includegraphics[width=.6\columnwidth]{./figs/GAA_conflict_graph_ex2}}
%	\caption{(a) Node-based conflict graph. (b) NC-pair conflict graph.
%		Available channels and demands for each CBSD are as follows: $\Gamma(A) = \{2,3\}$, $\mathcal{D}(A)=\{1,2\}$; $\Gamma(B)=\{1,2\}$, $\mathcal{D}(B)=\{1\}$; $\Gamma(C)=\{1,2\}$, $\mathcal{D}(C)=\{1\}$; and $\Gamma(D) = \{3,4,5\}$, $\mathcal{D}(C)=\{2,4\}$.
%		B and C are within each other's CS/ED range, and thus are able to coexist on CH 1 or 2. }
%	\label{fig:GAA_conflict_graph_ex}
%\end{figure}

%\begin{figure}[ht!]
%    \centering
%    \begin{subfigure}[b]{.25\columnwidth}
%    		\centering
%        \includegraphics[width=1\textwidth]{./figs/GAA_interference_graph_ex}
%        \caption{}
%        \label{fig:GAA_interference_graph_ex}
%    \end{subfigure}
%    ~ 
%    \begin{subfigure}[b]{.6\columnwidth}
%    		\centering
%        \includegraphics[width=1\textwidth]{./figs/GAA_conflict_graph_ex2}
%        \caption{}
%    \end{subfigure}
%    \caption{(a) Node-based conflict graph.
%    (b) NC-pair conflict graph.
%   	Available channels and demands for each CBSD are as follows: $\Gamma(A) = \{2,3\}$, $\mathcal{D}(A)=\{1,2\}$; $\Gamma(B)=\{1,2\}$, $\mathcal{D}(B)=\{1\}$; $\Gamma(C)=\{1,2\}$, $\mathcal{D}(C)=\{1\}$; and $\Gamma(D) = \{3,4,5\}$, $\mathcal{D}(C)=\{2,4\}$.
%     B and C are within each other's CS range, and thus are able to coexist on CH 1 or 2. }
%    \label{fig:GAA_conflict_graph_ex}
%\end{figure}


%\subsubsection{Example}
%Fig.~\ref{fig:GAA_conflict_graph_ex} is an example of a conflict graph for GAA channel assignment, derived from the following requests: 
%\begin{itemize}
%\item $\Gamma(A) = \{2,3\}$, $D(A)=\{1,2\}$;
%\item $\Gamma(B)=\{1,2\}$, $D(B)=\{1\}$; 
%\item $\Gamma(C)=\{1,2\}$, $D(C)=\{1\}$; and
%\item $\Gamma(D) = \{3,4,5\}$, $D(C)=\{2,4\}$.
%\end{itemize}
%When assigned to the same channel, A, B and C will conflict with each other; D will conflict with A, but not with B or C.
%As we can see, the conflict graph may also be generalized to account for pairwise adj-channel interference.
%
%\begin{figure}[ht!]
%    	\centering
%    	\includegraphics[width=0.6\columnwidth]{./figs/GAA_conflict_graph_ex}
%    \caption{Conflict graph example for GAA channel assignment. 
%    Edges \protect\circled{1} and \protect\circled{2} indicate the one-channel-assignment-per-radio and co-channel interference constraints, respectively.
%    }
%    \label{fig:GAA_conflict_graph_ex}
%\end{figure}


\subsubsection{Rewards}
In GAA CA, \rev{the basic objectives of the SAS} would include accommodating more nodes and \rev{assigning more channels.} %improve spectrum utilization. 
As a result, NC pairs that assign more channels to more nodes are generally more preferred. 
To reflect such preference, the SAS can define a \textit{reward (or vertex weighting) function} $R: V \mapsto \mathbb{R}^+$ that assigns a positive reward to each vertex $v=(S,C)$. 
\rev{If the SAS aims to meet more demand by assigning more channels,} the \textit{linear} reward function $R(v)=R(S,C) = |S|\cdot|C|$ may be used, which \rev{is equal to} the \rev{total} number of assigned channels \rev{at each vertex}. 
\rev{If the SAS wants to prioritize the objective of accommodating more nodes,} an alternative \textit{log} reward function \rev{may be adopted, i.e.,} $R(v)=R(S,C) = |S| \cdot ( 1 + \log(|C|))$, which captures the decreasing benefit of a node getting additional channels. 
%We call the above two reward functions \textit{linear} and \textit{log} reward functions, respectively. 

%In \cite{cao2005distributed}, the reward represents the maximum bandwidth/throughput that user(s) $S$ can acquire through channel $C$. 


\noindent \textbf{Problem Formulation}:
Given a vertex-weighted conflict graph $G(V,E,R)$ for $n$ nodes \rev{for binary GAA CA}\footnote{\rev{In this work, we focus on the CBSD-centric graph representation and algorithms for GAA CA. Hence, since GAA nodes are at fixed locations, the SAS does not need to consider node mobility. We will leave extending this work to client-centric and studying the impact of end user device mobility on the proposed algorithms as future work.}}, the SAS wants to find a scheme $I \subseteq V$ so as to \revv{maximize the total reward and accommodate more nodes, subject to the conflict constraint, i.e.,}
%maximize the total reward, subject to the cardinality and conflict constraints, i.e.,
%\begin{equation*}
%\max_{I \subseteq V} R(I), \text{ s.t. } \sum_{v\in I}|S(v)|=n;~ e(u,v) \notin E, \forall u,v \in I, \nonumber \label{eq:min_demand_max_reward_CA}
%\end{equation*}
%where $R(I)=\sum_{v\in I} R(v)$ is the total reward, and $S(v)$ is the set of nodes at vertex $v$. 
%
%In cases where the demand exceeds the supply, i.e., there are many more nodes than available channels, the SAS may not obtain a feasible solution to the above problem. 
%Hence, the SAS may relax it to the following optimization problem. 
%
%\noindent\textbf{Relaxed Problem Formulation}: 
%Given a vertex-weighted conflict graph $G(V,E,R)$, the SAS wants to find a scheme $I \subseteq V$ so as to \rev{maximize the total reward subject to the conflict constraint,}
%\begin{align}
%\max_{I \subseteq V}R'(I), \text{ s.t. }~ e(u,v) \notin E, \forall u,v \in I, 
%\label{eq:max_reward_CA}
%\end{align}
%where $R'(I)=\sum_{v\in I} (R(v) + \lambda |S(v)|)$ and $\lambda \geq 0$ is the trade-off parameter chosen by the SAS.
%\revv{Intuitively, the SAS aims to assign as many channels and serve as many nodes as possible
%at the same time.}
%We refer to the problem in (\ref{eq:max_reward_CA}) as \textbf{Max-Reward CA}.
\begin{align}
\max_{I \subseteq V} &~ R'(I) \nonumber \\ \text{Subject to: } e(u,v) &\notin E, \forall u,v \in I, 
\label{eq:max_reward_CA}
\end{align}
%\begin{align}
%\max_{I \subseteq V} R'(I)\text{, s.t. } e(u,v) &\notin E, \forall u,v \in I, 
%\label{eq:max_reward_CA}
%\end{align}
\revv{where $R'(I)=\sum_{v\in I} (R(v) + \lambda |S(v)|)$ ($S(v)$ is the set of nodes at vertex $v$) and $\lambda \geq 0$ is the trade-off parameter chosen by the SAS.}
We refer to the problem in (\ref{eq:max_reward_CA}) as \textbf{Max-Reward CA}.

%It is actually a generalization of the PA-CA problem formulation in Eq.~(\ref{eq:PA_CA_formulation}). 

\subsection{Conflict Graph with Non-Binary Conflicts for GAA CA }
%The previously proposed binary conflict graph exploits type-II conflicts. 
\rev{In order to} further exploit type-I conflicts, we extend the proposed conflict graph to \rev{incorporate} non-binary conflicts and formulate the CA problem as a utility maximization problem.
We start with a conflict graph without any super-NC pair as constructed in Section~\ref{sec:conflict_graph_binary}. 
To differentiate the impacts of a conflict on two interfering nodes, we consider directed edges and use a \textit{penalty (or edge weighting) function} $P: E \mapsto \mathbb{R}^+$ to assign a non-negative penalty to each directed edge.
Let the penalty of $e(u,v) \in E$  as $P(e(u,v))$ or simply $P_{u,v}$, i.e., \rev{the penalty on $v$ due to the interference from $u$.}
%the interference from $u$ to $v$.
In general, we have $P_{u,v} \neq P_{v,u}$, and $P_{u,v}=0$ if $e(u,v) \notin E$. 

%To quantify penalties, many existing measurement and modeling techniques can be deployed. For example, in \cite{padhye2005estimation}, Padhye \textit{et al.} defines the link interference ratio as the penalty, i.e., the ratio of aggregate output of the links when they are active simultaneously, to the aggregate throughput when they are active individually. This penalty can be empirically measured via broadcast probes.  In \cite{reis2006measurement}, Rei \textit{et al.} improves the scalability of the previous approach by developing an interference model based on RSSI measurements. In \cite{mishra2005weighted}, the penalty is defined as the number of clients associated with two interfering nodes that are affected if the two nodes are assigned the same channel. \rev{Due to the ease of practical implementation,} we use the interference estimated from a radio propagation model as penalty as in \cite{subramanian2007fast, kim2015design} in this work.

\begin{figure}[!t]
	\centering
	\includegraphics[width=.8\columnwidth]{./figs/GAA_modified_conflict_graph}
	\caption{
		Example of NC-pair conflict graph with non-binary conflicts.
		Each vertex \rev{is associated with} a reward and each directed edge has a penalty. 
		\rev{Note that NC pairs belonging to the same node are grouped as a cluster and there are no intra-cluster edges.}
		%There are no intra-cluster edges, and penalties for edges connecting NC pairs from the same super-NC pair are zero. 
	}
	\label{fig:GAA_modified_conflict_graph}
\end{figure}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.8\columnwidth]{./figs/GAA_modified_conflict_graph}
%%	\includegraphics[width=0.6\columnwidth]{./figs/GAA_modified_conflict_graph}
%    \caption{Example of a vertex- and edge-weighted conflict graph.
%    Each vertex has a reward, and each directed edge has a penalty value. 
%    Besides, there are no intra-cluster edges, and penalties for edges connecting NC pairs that form the same super-NC pair are $0$. }
%    \label{fig:GAA_modified_conflict_graph}
%\end{figure}


Fig.~\ref{fig:GAA_modified_conflict_graph} illustrates the proposed non-binary conflict graph.
In addition to the directed edges with penalties, the other main difference is that 
%, and there are two key differences, in addition to directed edges with penalties. First, 
the set of NC pairs that belong to the same node are grouped as a cluster, and there are no edges within a cluster.
The one-channel-assignment-per-node constraint is enforced instead by selecting at most one NC pair from each cluster. 
%Second, after super-NC pairs are identified, they are not added to the graph; instead, the penalties between two NC pairs that are associated with the same super-NC pair are set to zero.

\noindent \textbf{Problem Formulation}: 
Given a vertex-weighted and edge-weighted conflict graph $G(V,E,R,P)$ for $n$ nodes \rev{for non-binary GAA CA}, the SAS wants to find a scheme $I \subseteq V$ so as to 
\begin{align}
\max_{I \subseteq V} &~U(I) \nonumber \\
\text{Subject to: } |I \cap V_i| &\leq 1, \forall i=1,2,...,n, \label{eq:max_utility_CA}
\end{align}
%\begin{align}
%\max_{I \subseteq V} U(I) \text{, s.t. } |I \cap V_i| &\leq 1, \forall i=1,2,...,n, \label{eq:max_utility_CA}
%\end{align}
where 
\begin{equation}
U(I) = \sum_{v \in I} R(v) - \lambda \cdot \sum_{u,v\in I} P_{u,v} \label{eq:utility_function}
\end{equation}
is the \textit{utility function} and $\{V_i\}$ are NC-pair clusters that form a partition of $V$, that is, $V=\bigcup_{i}V_i$ and $V_i\cap V_j = \emptyset$ for $i\neq j$.
We refer to the above problem as \textbf{Max-Utility CA}.


==> ArXiv Submission/sections/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we \rev{studied SAS-assisted dynamic CA for the 3.5 GHz band.}
We proposed NC-pair conflict graph to model pairwise interference, spatially varying channel availability and channel contiguity. 
We further introduced super-NC pairs to exploit coexistence opportunities under type-II conflict and proposed the super-node formation algorithm to identify super-nodes.
The proposed conflict graph enables us to formulate PA CA as max-cardinality CA and GAA CA with binary conflicts as max-reward CA.
%, and further map them to the classic maximum (weighted) independent set problem. 
We adopted a heuristic-based algorithm to obtain approximate solutions.
To further enhance coexistence awareness, we extended binary conflicts to non-binary by assigning each conflict a penalty.
Then we formulated non-binary GAA CA as utility maximization. 
We showed that the utility function is submodular and  our problem is an instance of matroid-constrained submodular maximization. 
We proposed a local-search-based polynomial-time algorithm for max-utility CA that provides a provable performance guarantee. 
%an optimality guarantee of $1/4$. 

Our simulation results based on a real-world dataset show that the proposed max-cardinality algorithm consistently serves over $93.0\%$ of service areas and outperforms the baseline algorithm by over $30.0\%$ for PA CA.
For binary GAA CA, the proposed max-reward algorithm with linear rewards can accommodate $10.2\%$ more nodes and serve $10.4\%$ more demand on average than the baseline, and coexistence awareness can effectively improve the performance of the proposed algorithm.
For non-binary GAA CA, the proposed max-utility algorithm achieves $29.5\%$ more utility with much less total interference as compared to \revv{random selection}.
\revv{We also show that an operator can leverage the proposed framework to optimize the overall capacity of GAA networks.}






==> ArXiv Submission/sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
We \res{implemented} the proposed algorithms in MATLAB and compare their performance against baseline algorithms through extensive simulations. 
A real-world Wi-Fi hotspot location dataset in the New York City \cite{NYCWiFiLocation} is used to simulate \rev{a dense outdoor scenario}. Our results demonstrate the advantages of the proposed graph representation and algorithms for dynamic CA in the CBRS.


\subsection{Evaluation of Max-Cardinality CA}
For PA CA, we evaluate the proposed algorithm based on GMWIS (Algorithm~\ref{algo:GWMIS}) and compare it against a baseline algorithm called Non-Preemptive Sum Multi-Coloring (npSMC) \cite{bar2000sum}.
\res{To the best of our knowledge, npSMC is the only existing algorithm that explicitly considers channel contiguity, applicable to the PC CA scenario in the CBRS band.}


\subsubsection{Baseline}
The algorithm npSMC was proposed in \cite{bar2000sum} for scheduling dependent jobs on a graph, where each vertex $v$ is a job with a length or execution time $x(v)$ (i.e., required number of colors) and each edge indicates two dependent jobs that cannot be scheduled at the same time. 
Given a certain amount of time units or colors, the objective is to color as many vertices as possible, such that each vertex is assigned a desired amount of distinct contiguous colors and adjacent vertices are assigned disjoint sets of colors.

Given a graph $G(V,E,x )$, npSMC first puts vertices of the same length to the same group by adding an edge for each pair of vertices of different lengths, that is, $E'=E\cup \{(u,v):x(u)\neq x(v)\}$. 
This ensures that at any given time, vertices from the same group are being colored. 
Then it finds a maximal independent set (e.g., Algorithm~\ref{algo:GWMIS}) in the new graph $G'=(V,E')$ and color the selected jobs to completion non-preemptively 
in each iteration, until colors are exhausted.

\subsubsection{Setup}
We consider a square area of width $m$ that consists of $m^2$ census tracts, as shown in Fig.~\ref{fig:example_tract_topo}.
We generate randomly located circular areas of radius $r_s$ and consider census tracts that overlap with a circular area as a service area for PA CA purposes.
%Therefore, a larger $r_s$ means that more census tracts are likely to be included in a single service area.
The number of PALs \rev{held by the same PA licensee} for each service area is uniformly selected from $[1,4]$ at random. 
To simulate the worst case, we generate as many service areas as possible (up to $1000$ trials) subject to the seven-PALs-per-census-tract limit. 
Since the maximum possible size of a solution $I$ is equal to the total number of service areas $n$, we use the metric called \textit{ratio of service areas served}, $p=|I|/n$ to measure the performance for PA CA.


\begin{figure}[ht!]
	\vspace{-0.3cm}
	\centering
	\subfloat[]{\includegraphics[trim=0 .5cm 0 0,clip=true,width=.5\columnwidth]{./figs/matlab_figs/tract_topo_radius_0_5_width_5_seed_0}
		\label{fig:example_tract_topo}}
	\subfloat[]{\includegraphics[trim=0 -2cm 0 0,clip=true,width=.46\columnwidth]{./figs/NYC_WiFi_locations}
		\label{fig:NYC_WiFi_locations}}
	\caption{(a) Example of census tracts for PA CA. The set of census tracts that overlap with a red circle are treated as a service area for a PA licensee. In this example, each circle is of radius $0.4$ and each service area contains up to four census tracts. (b) Examples of Wi-Fi hotspot locations in NYC treated as CBSDs locations for GAA CA. In this example, there are $190$ GAA CBSDs inside the circle centered at the (randomly selected) location $(40.74,-73.99)$ with a radius of $1$ km. }
	%\vspace{-0.3cm}
\end{figure}

\subsubsection{Results}
To \rev{simulate} cities of different sizes, we set $r_s$ to $1$ and vary $m$ from $5$ to $30$ with a step of $5$.
For instance, with an optimal size of $4,000$ people for a census tract, $100$ census tracts ($m=10$) corresponds to a medium-sized city.
As mentioned in Section \ref{sec:PA_channel_assignment}, there are a total of $10$ PAL channels. 
Results are averaged over $100$ iterations. 
In each iteration, the same seed is used for the baseline and proposed algorithms for fair comparison. 

\begin{figure}[!t]
	\centering
	\subfloat[]{\includegraphics[trim=0 -.5cm 0 0,clip=true,width=.47\columnwidth]{./figs/matlab_figs/PA_CA_impact_of_area_width}
		\label{fig:PA_CA_impact_of_area_width}}
	\subfloat[]{\includegraphics[width=.49\columnwidth]{./figs/matlab_figs/PA_CA_impact_of_radius}
		\label{fig:PA_CA_impact_of_radius}}
%	\subfloat[]{\includegraphics[width=.3\columnwidth]{./figs/matlab_figs/PA_CA_impact_of_num_of_PAL_chns}
%		\label{fig:PA_CA_impact_of_num_of_PAL_chns}}
	\caption{Performance of the proposed and baseline algorithms vs. (a) area width and (b) radius. %, and (c) number of PAL channels.
	\revv{The proposed algorithm consistently serves over 93.0\% of the PA demands for different area widths and radii with significant improvements over the baseline algorithm.}
	}
	\label{fig:PA_CA_result}
	%\vspace{-0.3cm}
\end{figure}

As shown in Fig.~\ref{fig:PA_CA_impact_of_area_width}, the proposed algorithm serves $93.7\%$ of service areas on average, as compared to $70.1\%$ achieved by npSMC, with an improvement of $33.7\%$. 
We observe that due to the grouping in npSMC, service areas with larger demands tend to have lower priorities and thus often obtain no channels, whereas the proposed algorithm considers all service areas equally.

We then set $m$ to $10$ and vary $r_s$ from $0.4$ to $1.4$.
%vary the radius $r_s$ from $0.4$ to $1.4$, and each $r_s$ value (e.g., $1$) leads to service areas of various sizes (e.g., $3$ to $9$ census tracts).
%We set $m$ to $10$, and keep the rest the same. 
%As shown in Fig.~\ref{fig:PA_CA_impact_of_radius}, we can see that the proposed algorithm achieves $94.3\%$ on average, much better than that of the baseline, which is $71.4\%$ on average, with an improvement of $32.0\%$. 
\rev{As shown in Fig.~\ref{fig:PA_CA_impact_of_radius}, the average $p$ is $94.3\%$ and $71.4\%$ for the proposed algorithm and npSMC, respectively. The improvement is as high as $32.0\%$. }
%Although the number of PAL channels is $10$ according to FCC rules \cite{fcc2016}, we vary the number from $7$ to $12$ to study its impact. 
%The area width and radius are set to $10$ and $1$, respectively. 
%As illustrated in Fig.~\ref{fig:PA_CA_impact_of_num_of_PAL_chns}, if there are only $7$ PAL channels, $78.0\%$ of service areas are served using the proposed algorithm, as compared to $98.2\%$ with $12$ PAL channels;
%the performance is much worse using the baseline algorithm, which is $57.3\%$ and $78.8\%$, respectively.
%To conclude, with $10$ PAL channels,  the proposed algorithm is able to consistently meet more than $93.0\%$ of PA demands, irrespective of census tract topologies and service area sizes.
%With the proposed generic graph representation, more sophisticated algorithms for solving MWIS can be readily deployed, and we would expect the performance to increase. 
\rev{To summarize, our results show that the proposed algorithm is able to consistently meet more than $93.0\%$ of PA demands with a significant improvement over the baseline algorithm.}


\subsection{Evaluation of Max-Reward CA} \label{sec:evaluation_max_reward_CA}
In this section, we evaluate the proposed algorithm (Max-Reward) based on GMWIS (Algorithm~\ref{algo:GWMIS}) \rev{for binary GAA CA and compare it against the Max-Revenue Algorithm (MRA) in \cite{subramanian2008near}.}
%To the best of our knowledge, MRA is the only existing algorithm applicable to GAA CA with binary conflicts under the channel contiguity constraint.
Note that npSMC is not applicable, \rev{as it requires the same set of contiguous available channels at each node and cannot handle flexible demands.} 
We also evaluate the proposed algorithm %compare max-reward CA algorithms 
with different settings \rev{to study the impact of reward function and coexistence awareness.}
%i.e., with linear/log rewards and with/without coexistence-awareness. 

\subsubsection{Baseline} 
\res{MRA was proposed for bidding-based spectrum allocation in \cite{subramanian2008near}. It selects a set of non-conflicting NC pairs %with non-interfering nodes and non-overlapping channels, 
so as to maximize the total revenue, which corresponds to the total reward in our case. 
It is a greedy algorithm that iteratively selects the next non-conflicting NC pair with the maximum  incremental revenue. 
Note that MRA is coexistence unaware and its performance is not affected by the choice of the reward function.}

\subsubsection{Setup}
\rev{We consider a scenario where the SAS is serving a circular region of radius $r$ (in km) that is randomly located in the densely populated Manhattan area of NYC, as illustrated in  Fig.~\ref{fig:NYC_WiFi_locations}.}
\rev{We import outdoor Wi-Fi hotspot locations within the circular region from a publicly available dataset \cite{NYCWiFiLocation} and treat them as GAA nodes.
	
In order to create location-dependent channel availability for GAA nodes, we consider two PA licensees that are assigned with CH $1$-$4$ and CH $5$-$7$, respectively, and generate $10$ randomly deployed PA nodes for each licensee.}
\rev{A channel is considered available for a GAA node, if its $-80$ dBm/$10$ MHz interference contour\footnote{Strictly speaking, $-80$ dBm/$10$ MHz is the limit for the aggregate co-channel interference, and a lower limit may be chosen for pairwise co-channel interference. Nevertheless, the choice of this limit does not affect our evaluation, since the same set of available channels are used as input for both the proposed and baseline algorithms. } does not overlap with any PA node's default PPA (Section \ref{sec:PA_channel_assignment}).}
%The set of available channels for a GAA node are determined based on the criteria in Section~\ref{sec:PA_channel_assignment}, and the number varies from $8$ to $15$, depending on location.
%For simplicity, w
\rev{Each GAA node has a demand set $\mathcal{D}=\{1,2,3,4\}$ and an activity index $\alpha$ in $U[0,4]$.} 
\revv{In this work, we adopt the PA interference protection rules for determining the interference relationship between two GAA nodes, that is,}
a GAA node $j$ is said to be interfering with $i$, if its interference at a location inside $i$'s $-96$ dBm/$10$ MHz service contour 
is higher than $-80$ dBm/$10$ MHz. %(Section~\ref{sec:conflict_graph_binary}). 
The CS/ED threshold \rev{is set to $-75$ dBm/$10$ MHz (adapted from $-72$ dBm/$20$ MHz in \cite{etsi2016lte})}. 
%is between $-80$ and $-70$ dBm.
%\footnote{In \cite{80211ac2013}, the CS threshold for Wi-Fi signals is $-82$dBm/$20$ MHz
%In \cite{etsi2016lte}, the energy-detection threshold for LAA is considered to be $-75$ dBm/10 MHz, so it is reasonable to assume the range of $[-80, -70]$ dBm.}. 
The transmit power is $30$ dBm for each node, and transmit and receive antenna heights are $3$ and $1.5$ meters, respectively \cite{fcc2016}. 
We adopt the widely used COST-231 Hata \cite{damosso1999digital} as the propagation model.
Two metrics are adopted to measure the performance: 1) \textit{percentage of nodes served}, denoted as $p_1$,
and 2) \textit{percentage of demands served}, denoted as $p_2$, i.e., the ratio between the total number of assigned channels and the total demand. %(i.e., $4n$). 

\begin{figure}[!t]
	\centering
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_n_p1}
		\label{fig:max_reward_CA_impact_of_n_p1}}
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_n_p2}
		\label{fig:max_reward_CA_impact_of_n_p2}}
	\caption{Performance of the proposed and baseline algorithms in terms of average $p_1$ in (a) and $p_2$ in (b) as function of $n$. 
	\revv{The proposed algorithms outperform the baseline algorithm, and this advantage is further enhanced by coexistence awareness.}}
	\label{fig:max_reward_CA_impact_of_n}
	%\vspace{-0.3cm}
\end{figure}

\subsubsection{Results}
\rev{In order to study the performance of Max-Reward for regions with different sizes, we vary $r$ from $0.4$ km to $1.2$ km.
The trade-off parameter $\lambda$ and the sum activity index limit $\bar{\alpha}$ are set to $0$ and $1$, respectively. 
Results are averaged over $30$ iterations.}

\rev{As shown in Fig.~\ref{fig:max_reward_CA_impact_of_n}, the size of the SAS's service region does not have a significant impact on the performance of a CA algorithm.
Without coexistence awareness, Max-Reward-Linear and Max-Reward-Log  achieve an average $p_1$ larger than $72.6\%$ and $90.5\%$ in all cases and outperform the baseline algorithm by $10.2\%$ and $36.4\%$ on average, respectively. 

On the other hand, Max-Reward-Log has very close performance with the baseline algorithm in terms of average $p_2$, while Max-Reward-Linear outperforms the baseline  by $10.4\%$ on average. 
The above behaviors of Max-Reward are not surprising, since the log reward function encourages assigning a channel to nodes with fewer channels, leading to a larger $p_1$ but a smaller $p_2$.
	
We can also observe that coexistence awareness effectively improves the performance  of Max-Reward-Linear in terms of average $p_1$ by $11.7\%$ but has little effects on Max-Reward-Log. On the other hand, it is able to improve both Max-Reward-Linear and Max-Reward-Log in terms of average $p_2$ by $12.8\%$ and $17.4\%$ on average, respectively. }

\begin{figure}[!ht]
	\centering
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_lambda_p1}
		\label{fig:max_reward_CA_impact_of_lambda_p1}}
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_lambda_p2}
		\label{fig:max_reward_CA_impact_of_lambda_p2}}\\
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_alpha_limit_p1} \label{fig:max_reward_CA_impact_of_alpha_limit_p1}}
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_alpha_limit_p2} \label{fig:max_reward_CA_impact_of_alpha_limit_p2}}
	\caption{Impact of $\lambda$ and $\bar{\alpha}$ on the performance of the proposed algorithm in terms of average $p_1$ and $p_2$. 
	\revv{There exists a trade-off between $p_1$ and $p_2$ when choosing $\lambda$. 
	In addition, increasing $\bar{\alpha}$ can improve both $p_1$ and $p_2$, but such improvements no longer exist, when $\bar{\alpha}$ is large enough and all nodes in a clique are considered as a single super-node.}
	}
	\label{fig:max_reward_CA_impact_of_lambda}
	%\vspace{-0.3cm}
\end{figure}

\subsubsection{Impact of $\lambda$ and $\bar{\alpha}$} \rev{In order to study the impact of $\lambda$, we set $r=0.8$, $\bar{\alpha}=1$, and vary $\lambda$ from $0$ to $8$. 
As illustrated in Fig.~\ref{fig:max_reward_CA_impact_of_lambda_p1} and \ref{fig:max_reward_CA_impact_of_lambda_p2}, there exists a trade-off between $p_1$ and $p_2$ when choosing $\lambda$ for the proposed algorithm.
%With a larger $\lambda$, the algorithm puts more weight on the cardinality of the node set in each vertex, and  super-NC pair less likely to be selected.
With a larger $\lambda$, the proposed algorithm prioritizes the objective of serving more nodes by assigning more weight on the cardinality of the node set in each vertex, thus increasing $p_1$ but reducing $p_2$. 
We also see that that with a large $\lambda$, coexistence awareness does not help improve $p_1$ but is still able to effectively improve $p_2$.}

%Fig.~\ref{fig:max_reward_CA_impact_of_lambda} illustrates the impact of $\lambda$ with $n=200$.
%We can see that when $\lambda$ increases, the proposed algorithm is able to serve more nodes but fewer demands in all settings. 
%When $\lambda$ is $8$, all nodes are served, but only $48.2\%$ and $36.5\%$ of the total demand is met with linear- and log-reward coexistence-unaware max-reward CA, respectively, whereas coexistence awareness effectively increases $p_2$ to $58.3\%$ and $46.4\%$.
%This is not difficult to understand: from Eq.~(\ref{eq:max_reward_CA}), we can see that a greater $\lambda$ puts more value on the size of the node set in a NC pair, and thus a higher priority on $p_1$. 

%\begin{figure}[!ht]
%	\centering
%	\subfloat[]{\includegraphics[width=.4\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_cs_thr_p1} \label{fig:max_reward_CA_impact_of_cs_thr_p1}}
%	\subfloat[]{\includegraphics[width=.4\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_cs_thr_p2} \label{fig:max_reward_CA_impact_of_cs_thr_p2}}
%	
%	\subfloat[]{\includegraphics[width=.4\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_alpha_limit_p1} \label{fig:max_reward_CA_impact_of_alpha_limit_p1}}
%	\subfloat[]{\includegraphics[width=.4\columnwidth]{./figs/matlab_figs/max_reward_CA_impact_of_alpha_limit_p2} \label{fig:max_reward_CA_impact_of_alpha_limit_p2}}
%	\caption{Impact of CS/ED threshold and sum activity index limit ($\bar{\alpha}$) on the proposed coexistence-aware algorithm.}
%	\label{fig:max_reward_CA_impact_of_coexistence}
%\end{figure}

%\subsubsection{Coexistence Awareness}
%Fig.~\ref{fig:max_reward_CA_impact_of_coexistence} illustrates the impact of CS/ED threshold and sum activity index limit $\bar{\alpha}$ on the proposed algorithm with $n=200$ and $\lambda=0$.
%As the CS/ED threshold increases, $p_1$ and $p_2$ tend to decrease linearly for both linear- and log-reward CA, but its impact on $p_1$ for log-reward CA is the least. 
%On the other hand, when $\bar{\alpha}$ increases, the performance improves accordingly, but later saturates at $\bar{\alpha}=2$. 
%This is because when $\bar{\alpha}$ is large enough, all nodes in a clique will be considered as a super-node, at which point increasing $\bar{\alpha}$ does not help any more.

\rev{We then set $r=0.8$, $\lambda=0$ and vary $\bar{\alpha}$ from $0$ to $5$.
As shown in Fig.~\ref{fig:max_reward_CA_impact_of_alpha_limit_p1} and \ref{fig:max_reward_CA_impact_of_alpha_limit_p2}, a larger $\bar{\alpha}$ value allows more nodes to form a super-node, thus increasing both $p_1$ and $p_2$.
Nevertheless, such improvement tends to saturate at $\bar{\alpha}=2$, at which point all nodes in a clique are considered as a super-node and thus further increasing $\bar{\alpha}$ does not help any more.}


\subsection{Evaluation of Max-Utility CA}
%As shown in the previous section, one issue with max-reward CA is that not all nodes are assigned channels due to the binary nature of conflicts, especially when the network is crowded. 
%To address this issue, we formulate max-utility CA, and propose a polynomial-time algorithm based on matroid-constrained submodular maximization.  
In this section, we evaluate the proposed \revv{Max-Utility} algorithm (Algorithm~\ref{algo:UM_algorithm}) for non-binary GAA CA and compare its performance against a random selection-based baseline algorithm, which randomly selects a NC pair from each cluster. 
It repeats the process multiple times (e.g., $10000$) and returns the one with the maximum utility.

\subsubsection{Setup} 
We use the same setup in Section~\ref{sec:evaluation_max_reward_CA} and set $\epsilon=0$ for Algorithm~\ref{algo:UM_algorithm}. 
\revv{We consider two choices for reward and penalty functions.
In the first case, the number of channels assigned to each node is used as the reward, which is proportional to the best-case capacity %that can be achieved 
(no interference). As in \cite{subramanian2007fast, kim2015design}, the estimated interference %estimated from the radio propagation model 
is used as the penalty  (normalized by the maximum pairwise interference).

In the second case, we are interested in the overall capacity of GAA networks \cite{hessar2015capacity}. Suppose that vertices $v$ and $u$ are selected for nodes $i$ and $j$, respectively. 
Let the signal to noise and interference ratio of node $i$'s client at location $x$ in channel $c_k$ be $\text{SINR}_i(x,c_k)=\gamma_i^{(k)}(x)/(N_0 W_0 +\sum_{j\neq i} \gamma_{i,j}^{(k)}(x))$, where $N_0$ is the noise power density (Watts/Hz), $W_0=10$ MHz is the bandwidth of a GAA channel, and $\gamma_i^{(k)}(x)$ and $\gamma_{i,j}^{(k)}(x)$ are the received power (Watts) and the interference due to node $j$ (Watts) at location $x$ in channel $c_k$, respectively.  
Hence, the capacity in channel $c_k$ averaged over the service area $\mathcal{A}_i$ is $\bar{C}_i(c_k)= W_0 \int_{\mathcal{A}_i} \frac{\log_2 (1+ \text{SINR}_i(x, c_k))}{\mathcal{A}_i} d x$, and the overall capacity of a GAA network is the sum of capacities over all assigned channels, i.e., $\bar{C}_i = \sum_{c_k \in C(v)} \bar{C}_i(c_k)$, where $C(v)$ is the set of assigned channels at vertex $v$. 

We consider the best-case capacity (no interference) as the reward of vertex $v$, namely, $R(v)=\bar{C}_i$, where $\bar{C}_i=\sum_{c_k \in C(v)} W_0 \int_{\mathcal{A}_i} \frac{\log_2 (1+ \text{SINR}_i(x, c_k))}{\mathcal{A}_i} d x$ and $\text{SINR}_i(x, c_k)=\gamma_i^{(k)}(x)/(N_0 W_0)$.  
If vertex $u$ is also selected, the SINR at location $x$ will be $\text{SINR}_i(x,c_k)=\gamma_i^{(k)}(x)/(N_0 W_0 + \gamma_{i,j}^{(k)}(x))$ and let the resulting capacity be $\bar{C}_i'$ \footnote{We focus on the pairwise interference between GAA nodes and thus omit the interference from incumbents.}. 
The penalty on edge $e(u,v)$ is defined as the capacity reduction, i.e., $P(e(u,v))=\bar{C}_i-\bar{C}'_i$. 
Therefore, the utility (with $\lambda=1$) corresponds to the overall capacity under pairwise interference.
Nevertheless, the parameter $\lambda$ %in the utility function (Eq.~(\ref{eq:utility_function})) 
can be adjusted to account for the difference between the actual capacity and that under pairwise interference.}
%The linear reward function is used, and the interference normalized by the maximum pairwise interference is used as the penalty.
%\revv{The linear reward function is used and represents the number of channels assigned to each node, which is proportional to the best-case capacity that can be achieved in the absence of interference.}

%There are many options for penalties from literature.For example, Padhye \textit{et al.} defines the link interference ratio as the penalty \cite{padhye2005estimation}, that is, the ratio of aggregate output of the links when they are active simultaneously, to the aggregate throughput when they are active individually. This penalty can be empirically measured via broadcast probes.  
%%In \cite{reis2006measurement}, Rei \textit{et al.} improves the scalability of the previous approach by developing an interference model based on RSSI measurements. 
%In \cite{mishra2005weighted}, the penalty is defined as the number of clients associated with two interfering nodes that are affected if the two nodes are assigned the same channel. Due to the ease of practical implementation, we use the interference estimated from a radio propagation model as penalty as in \cite{subramanian2007fast, kim2015design} (normalized by the maximum pairwise interference) in this work.  
%\footnote{While the number of assigned channels is used as the reward and the estimated pairwise interference is chosen as the penalty in this work, our proposed algorithm is not limited to the chosen reward or penalty function. For example, the capacity averaged over client device locations \cite{hessar2015capacity} (assuming no interference, i.e., best-case) can be adopted as the reward, and the amount of capacity reduction due to the interference introduced by the conflicting node as the penalty. In this case, the total utility ($\lambda=1$) reflects the overall capacity under the pairwise interference relationship. Besides, $\lambda$ can be adjusted to account for the difference between the actual capacity reduction and the capacity reduction under pairwise interference.}. The performance is measured in terms of \rev{the achieved \textit{utility}} and \textit{the total amount of interference}.

%In this experiment, the same setup in Section~\ref{sec:evaluation_max_reward_CA} is used.
%We use linear reward function, and set CS/ED threshold and $\bar{\alpha}$ to $-75$ dBm and $4$, respectively. 
%The parameter $\epsilon$ in Algorithm~\ref{algo:UM_algorithm} is set to $0$.
%In addition to $p_1$ and $p_2$, we are also interested in \textit{the total amount of interference}. 
%The baseline is a greedy algorithm that starts with an empty set, and iteratively selects the NC pair with the maximum marginal utility subject to the matroid constraint, until the next NC pair is no longer beneficial (i.e., negative marginal utility). 

\begin{figure}[!t]
	\centering
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_utility_CA_impact_of_n_utility}\label{fig:max_utility_CA_impact_of_radius_utility}}
	\subfloat[]{\includegraphics[width=.49\columnwidth]{./figs/matlab_figs/max_utility_CA_impact_of_n_interference}\label{fig:max_utility_CA_impact_of_radius_interference}}
	\caption{Performance of \revv{Max-Utility and random selection} in terms of (a) averaged utility and (b) averaged total interference as a function of the radius of SAS's service region. \revv{Max-Utility achieves a much greater utility and smaller total interference than random selection.}}
	\label{fig:max_utility_CA_impact_of_radius}
\end{figure}

\subsubsection{Results}
\revv{In the first case,} we set $\lambda=1$ and vary the radius $r$ from $0.4$ km to $1.2$ km. Results averaged over $30$ iterations are provided in Fig.~\ref{fig:max_utility_CA_impact_of_radius}.
As we can see, \revv{Max-Utility} is able to achieve a much greater utility than \revv{random selection}, especially when SAS's service region becomes larger. The improvement in average utility is more than $29.5\%$ in all cases and reaches $50.2\%$ with $r=1.2$ km. 
Besides, \revv{Max-Utility generates smaller total interference than random selection and allows the SAS to serve almost all nodes and demands.}

\revv{The impact of $\lambda$ is illustrated in Fig.~\ref{fig:max_utility_CA_impact_of_lambda} with $r=0.8$ km.}
%\rev{In order to study the impact of $\lambda$, we set $r$ to $0.8$ and vary $\lambda$ from $10^0$ to $10^3$. Results averaged over $30$ iterations are shown in Fig.~\ref{fig:max_utility_CA_impact_of_lambda}.
We can observe that increasing $\lambda$ reduces the achieved utility, but the decrease for \revv{Max-Utility} is slower than \revv{random selection}. This is because a larger $\lambda$ implies a larger weight on the interference, which effectively makes \revv{Max-Utility} avoid selecting NC pairs with larger interference.
It also explains the decrease in the total interference for \revv{Max-Utility}. 
In all cases, \revv{Max-Utility} achieves a much greater utility while keeping the total interference much smaller than \revv{random selection}.

\begin{figure}[!t]
	\centering
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_utility_CA_impact_of_lambda_utility}\label{fig:max_utility_CA_impact_of_lambda_utility}}
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_utility_CA_impact_of_lambda_interference}\label{fig:max_utility_CA_impact_of_lambda_interference}}
	\caption{Performance of \revv{Max-Utility and random selection} in terms of (a) averaged utility and (b) averaged total interference as a function of the trade-off parameter $\lambda$. \revv{We can see that increasing $\lambda$ puts more weights on the interference, thus leading to less interference at the cost of reduced utility.}}
	\label{fig:max_utility_CA_impact_of_lambda}
	%\vspace{-0.4cm}
\end{figure}

\begin{figure}[!h]
	\centering
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_utility_CA_impact_of_radius_capacity}\label{fig:max_utility_CA_impact_of_radius_capacity}}
	\subfloat[]{\includegraphics[width=.48\columnwidth]{./figs/matlab_figs/max_utility_CA_impact_of_lambda_capacity}\label{fig:max_utility_CA_impact_of_lambda_capacity}}
	\caption{\revv{Average utility or capacity (Mbits/sec) achieved by Max-Utility and random selection as a function of the radius  $r$ and trade-off parameter $\gamma$. In both settings, Max-Utility leads to a much higher utility than random selection. }}
	\label{fig:max_utility_CA_capacity}
\end{figure}

\revv{In the second case, the same experiments are repeated and results are provided in Fig.~\ref{fig:max_utility_CA_capacity}. 
We observe that as $r$ increases, the average utility or capacity achieved by Max-Utility increases at a much faster rate than random selection. 
On the other hand, increasing $\lambda$ also increases the achieved utility, but Max-Utility significantly outperforms random selection.}



==> ArXiv Submission/sections/introduction.tex <==
\section{Introduction}
The rapidly increasing demand in wireless capacity with future ultra-broadband wireless networks 
is driving regulatory bodies to pursue policy innovations based on the paradigm of \textit{shared spectrum}. 
Such paradigm allows secondary devices to access licensed spectrum bands that are underutilized by primary owners.
In \cite{fcc2008TVWS}, the FCC allowed the unlicensed use of underutilized TV spectrum as a first step. 
In the 2012 PCAST report \cite{PCAST2012}, the U.S. government pushed it further by announcing its intentions to explore spectrum sharing policies and innovative technologies to share 1000 MHz federal government spectrum with commercial systems. 
Towards this goal, the FCC targeted \rev{the} release of 3550-3700 MHz band for small cell deployment, termed \rev{the} \textit{Citizens Broadband Radio Service} (CBRS), which is primarily used by high-power Department of Defense shipborne radars and non-federal Fixed Satellite Services (FSS) earth stations.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{./figs/3_tier_framework2}
    \caption{Three-tiered spectrum access in 3.5 GHz CBRS band. }
    \label{fig:three_tier_framework}
\end{figure}

%\subsection{A Spectrum Access Rights Perspective -- Three-Tiered Spectrum Management Framework}
In \rev{the} recent ruling \cite{fcc2012,fcc2014,fcc2015,winnforum2018requirements} for \rev{the} CBRS, the FCC proposed a spectrum \rev{access} framework that consists of three tiers: 1) \textit{Incumbent Access}, 2) \textit{Priority Access} (PA), and 3) \textit{Generalized Authorized Access} (GAA), as illustrated in Fig.~\ref{fig:three_tier_framework}. 
PA and GAA devices are also referred to as \res{Citizens Broadband Radio Service Devices (CBSDs), which are fixed stations or networks of such stations operating on a PA or GAA basis. End user devices are not considered as CBSDs.}
As we can see, the above framework highlights the hierarchical spectrum access rights: 
Incumbents have the highest priority and %, including authorized federal and FSS users,  
would be protected from harmful interference from all other users by forbidding %co-channel (and adj-channel) 
CBSD transmissions within and close to the \rev{activated \textit{Dynamic Protection Areas} (DPAs)}.
\rev{PA users with critical quality-of-service needs (e.g., hospitals and public safety entities) would be authorized to operate at specific locations with certain interference protection.} \rev{ %For this purpose, 
But they need to purchase} PA licenses (PALs) \rev{via competitive bidding}, each of which guarantees the authorized and protected use of a $10$ MHz channel in a census tract.
%Specifically, the co-channel interference from other PA or GAA devices cannot exceed $-80$ dBm/$10$ MHz within the \textit{PAL protection area} of a PA CBSD. 
In contrast, GAA CBSDs (or GAA nodes) would be authorized to %opportunistically 
access the shared bands within designated geographic areas, but they \rev{would expect no interference protection and should avoid causing interference to incumbents and PA users}. 
In the center of the CBRS ecosystem lies the \textit{Spectrum Access System} (SAS) \rev{that authorizes and manages use of spectrum for the CBRS.}
%that enforces incumbent protection, dynamically assigns and keeps track of real-time spectrum use.  
\rev{In this work, we study the SAS-assisted dynamic channel assignment (CA) for PA and GAA tiers.}

%In order to provide a flexible, scalable, practically deployable bandwidth for high data rate technologies,
The 3.5 GHz band is divided into $15$ orthogonal $10$ MHz channels. %(CH $1$-$15$). 
%As for PA CA, 
Up to $7$ channels can be assigned to PALs in a \textit{license area} (a census tract), %, and the actual channel for each PAL is assigned by the SAS.
%Spectrum aggregation is permitted but up to a limit to strike the balance between ensuring a diversity of users and allowing for applications that require larger blocks of spectrum. 
%Specifically, a 
and a licensee is allowed to aggregate up to $4$ channels by stacking multiple \revv{PALs} in a \textit{service area} (one or more contiguous license areas).
\rev{While each PAL guarantees one channel, the exact channel assignment is not fixed and will be determined by the SAS.}
Since the FCC requires the SAS to assign \textit{contiguous channels to geographically contiguous PALs}, it imposes a major challenge to the design of a PA CA scheme.

To improve spectrum utilization, a PAL channel is made available for GAA use at locations outside the \textit{PAL protection areas} (PPAs) and their vicinities under the ``use-it-or-share-it'' rule.
\rev{As a result}, \textit{channel availability} becomes location dependent and may vary significantly among GAA nodes.
Moreover, a GAA node may also request multiple \textit{contiguous channels} to meet its capacity demand or support network operations. 
For instance, a Wi-Fi-based node would require at least two contiguous channels in the CBRS. 

In this work, we are interested in co-channel coexistence enabled by Wi-Fi like MAC protocols, such as CSMA/CA \cite{80211ac2013} and Listen-Before-Talk in LTE-LAA \cite{etsi2016lte}. 
\rev{Hence,} the pairwise interference relationship of GAA nodes can be classified into three cases: 1) no conflict, 2) type-I conflict -- two interfering nodes are hidden from each other and cannot detect \res{possible interference at end user devices (or clients) without their feedbacks (e.g., packet loss or throughput degradation)}, \rev{or} 3) type-II conflict -- two interfering nodes are within each other's carrier-sensing (CS) or energy-detection (ED) range and can resolve the conflict through contention. %without feedback \rev{from end user devices}. 
Since GAA nodes are able to harmoniously share the same channel under type-II conflicts, %with low overhead, 
the SAS \rev{can} exploit such \textit{coexistence opportunities} to accommodate more devices \rev{in a dense network}.

%
%%\subsection{An Inter-Technology Coexistence Perspective}
%In the GAA tier, the equal priority access nature requires  unlicensed devices and networks that deploy different radio access technologies (RATs) by different operators to \textit{coexist} in the same frequency, time and space.
%Wi-Fi and LTE are the two most prominent RATs being deployed today and promising candidates for the CBRS band. 
%Intra-RAT coexistence among Wi-Fi networks is enabled by Carrier Sensing Medium Access with Collision Avoidance (CSMA/CA),
%which is a contention based listen-before-talk (LBT) mechanism, where each device senses the medium and allow other devices to finish transmission before attempting its own transmission.
%In contrast, traditional LTE does not sense the medium before transmission, and the deployment of LTE networks in the same band (typically managed by the same operator) is usually planned and exploits spatial frequency reuse.
%Due to the difference in MAC layer mechanisms, co-channel coexistence between Wi-Fi and LTE networks is problematic and unavoidably leads to degraded performance (especially for Wi-Fi networks) \cite{cavalcante2013performance}.
%
%MAC layer time-sharing mechanisms are a key enabler for harmonious inter-RAT co-channel coexistence between Wi-Fi and LTE.
%In some regions like Europe, Japan and India, Wi-Fi like LBT mechanisms \cite{ratasuk2012license, qualcomm2014lte} have been become regulatory requirement, 
%while in other regions like US, China and South Korea, LBT is not required phase-wise for early commercialization, and non-LBT mechanisms based on duty cycles are proposed, which require LTE radios to transmit for a fraction of time and create gaps for radios deploying other RATs to transmit.
%Examples include carrier-sensing adaptive transmission (CSAT) \cite{qualcomm2014lte}, almost blank subframes \cite{almeida2013enabling}, muting \cite{nihtila2013system} and subframe puncturing \cite{qualcomm2015lteU}.
%Recently, coordinated time division channel access was proposed in \cite{sagari2015coordinated}, where networks of each RAT take turns to access the channel.


%\begin{figure*}[ht!]
%    \centering
%    \includegraphics[width=0.8\textwidth]{./figs/overall_system_arch}
%    \caption{End-to-end architecture for the CRBS band.}
%    \label{fig:overall_system_arch}
%\end{figure*}

Despite that dynamic CA has been studied in the context of spectrum sharing from various perspectives such as graph coloring \cite{mishra2005weighted, subramanian2007fast, subramanian2008near, hessar2014resource} and
%pricing \cite{niyato2008competitive} 
game theory \cite{nie2006adaptive,liu2008spectum,
li2012distributed},
the aforementioned challenges (i.e., channel and geographic contiguity, spatially varying channel availability, and coexistence \rev{awareness}) differentiate dynamic CA in the CBRS from previous work. 
%In this paper, we focus on SAS-assisted
%closed-loop\footnote{It differs from the open-loop model, in which SAS plays ``an advisory role'' in improving channel management and interference by providing a list of ranked channels by certain performance metrics \cite{kim2015design}.} 
%CA for PA and GAA tiers and address the above challenges with graph and combinatorial theories.
%Our primary contributions are as follows:
In this paper, we make the following specific  contributions:
\begin{itemize}
\item We define the \textit{node-channel pair} (NC pair) that assigns a set of contiguous and available channels to a node (i.e., a PA service area or a GAA CBSD) and introduce the \textit{NC-pair conflict graph}, in which each vertex is a NC pair and each edge represents a conflict. 

\item With the proposed conflict graph, we formulate PA CA as \textit{max-cardinality CA}. 
For GAA CA with binary conflicts, we extend NC pairs to \textit{super-NC pairs} to exploit type-II conflicts, where each super-node consists of a set of GAA nodes that can detect each other's transmission.
We define a reward function to capture the preferences of (super-)NC pairs and formulate binary GAA CA as \textit{max-reward CA}. 
To further enhance coexistence awareness, %exploit type-I conflicts, 
we define a penalty function and extend the binary conflicts to non-binary.
The non-binary GAA CA is then formulated as \textit{max-utility CA} to trade off rewards against penalties.

\item We propose a super-node formation algorithm based on clique searching and bin packing. % to identify super-nodes.
The max-cardinality and max-reward CA problems are mapped to the problem of finding the maximum (weighted) independent set, and approximate solutions are obtained through a heuristic-based algorithm.
For max-utility CA, we show that the utility function is submodular, and our problem is an instance of matroid-constrained submodular maximization.
% in combinatorial theory.
We propose a polynomial-time algorithm based on (approximate) local search that provides a provable performance guarantee. 

\item We conduct extensive simulations \rev{using a real-world dataset that contains Wi-Fi hotspot locations in the New York City} \cite{NYCWiFiLocation} to evaluate the proposed algorithms.
For PA CA, our results show that the proposed algorithm consistently serves over $93.0\%$ of service areas and outperforms the baseline algorithm by over $30.0\%$.
For binary GAA CA, the proposed algorithm with linear rewards \rev{is able to accommodate $10.2\%$ more nodes and serve $10.4\%$ more demand on average than the baseline algorithm}. \rev{Besides, enabling coexistence awareness can effectively improve the performance of the proposed algorithms}. 
For non-binary GAA CA, \rev{the proposed algorithm achieves $29.5\%$ more utility while keeping the total interference much smaller than \revv{random selection}}.
\revv{We also show that an operator can leverage the proposed framework to optimize the overall capacity of GAA networks.}
% in the presence of pairwise interference



%We conduct extensive simulations on networks built on a real WiFi AP topology in NYC. 
%We compare our algorithms against a baseline algorithm  \cite{hessar2014resource} in simplified settings, and further evaluate our algorithms in more general settings.
%Our results show that min-/max-demand CA achieves very close performance with the baseline, but handles multi-channel demands with the channel contiguity constraint much better.
%Besides,  max-demand CA allocates more channels but accommodate fewer radios, while min-/max-demand CA is able to accommodate more radios. 
%Furthermore, coexistence effectively helps SAS to allocate more channels to more radios, and such benefits are more significant in denser networks. 

\end{itemize}

The remainder of this paper is organized as follows.
Section~\ref{sec:related_work} reviews the related work on CA.
Section~\ref{sec:channel_assignment_scenario} summarizes CA scenarios and presents the SAS-based architecture.
Conflict graphs and problem formulations are presented in Section~\ref{sec:conflict_graph}, and proposed algorithms are provided in Section~\ref{sec:algo}.
Section~\ref{sec:evaluation} presents simulation results and Section~\ref{sec:conclusion} concludes this study.






==> ArXiv Submission/sections/preliminaries.tex <==
\section{Preliminaries}
In this section, we briefly review some concepts in graph theory and introduce notations that will be used throughput this paper. 
We also provide background on the one-dimensional bin-packing problem and submodularity. 

\subsection{Review on Graph Theory}
Let $G=(V,E,W)$ be a weighted undirected graph without loops and multiple edges, where $V$ is the set of verties, $E$ is the set of edges, and $W$ is the vertex weighting function such that $W:2^V\mapsto \mathbb{R}^+$. 
For any nonempty set $S\subseteq V$, $W(S) = \sum_{u \in S} W(u)$ is the weight of $S$. 

We use $V(G)$ and $E(G)$ to denote the set of vertices and edges in $G$, and use $e(u,v)$ to denote the edge that connects vertices $u,v\in V$. 
Let $G[V']$ be the subgraph of $G$ induced by $V'$, $\delta_G(v)$ the degree of vertex $v$, and $\Delta_G$ the maximum degree of $G$. 


\begin{mydef}[(Maximum) Independent Set (IS)]
Given a weighted undirected graph $G=(V,E,W)$, a subset $I \subseteq V$ is an \textit{independent set} of $G$ if for any two vertices $u,v \in I$, $e(u,v) \notin E$. 
An independent set $I$ of $G$ is \textit{maximum} if there is no independent set $I' \neq I$ of $G$ such that $W(I) < W(I')$.
\end{mydef}

The \textit{maximum weighted independent set} (MWIS) problem is to find the maximum independent set. 
When each vertex has an equal weight of $1$ (i.e., unweighted), it becomes the MIS (maximum independent set) problem.
As one of most important NP-hard problems \cite{halldorsson2000approximations}, there are no efficient algorithms in sight for MWIS, and heuristic methods (e.g., greedy strategies) are often used to obtain an approximate solution with certain performance guarantee. 
Denote the weight of a maximum IS of $G$ by $\theta(G)$, and the weight of the solution obtained by algorithm $A$ by $A(G)$.
The \textit{performance ratio} is defined by $\rho_A = \inf_G \frac{A(G)}{\theta(G)}$.

\begin{mydef}[(Maximal) Clique]
Given an undirected graph $G=(V,E)$, a subset $S\subseteq V$ is a clique of $G$, if for any two $u,v\in S$, $e(u,V)\in E$.
A clique is maximal if it cannot be extended by including one more adjacent vertex. 
\end{mydef}

\subsection{One-Dimensional Bin-Packing Problem}
The classic one-dimensional bin-packing problem \cite{coffman1978application,eilon1971loading,dosa2007tight, coffman1996approximation} is as follows: given $n$ items with sizes $s_1,s_2,...,s_n \in \mathbb{R}^+$, we want to find the smallest number of bins, each having a capacity of $C$, such that each item is packed into exactly one of the bins, and the sum of the sizes of the items in each bin is no more than $C$. 
It is well known that the bin-packing is NP-hard \cite{coffman1978application}, and algorithms based on heuristics such as the First Fit Decreasing algorithm \cite{eilon1971loading,dosa2007tight} are often used to find near-optimal solutions. 
A comprehensive survey on this topic is available in \cite{coffman1996approximation}.


\subsection{Submodularity}\label{sec:submodularity}
Submodularity is a property of set functions that captures the \textit{diminishing returns} behavior, that is, adding a new element introduces greater incremental benefits, if there are fewer elements so far, and less, if there are more elements.  
The formal definition is the following.

\begin{mydef}[Submodularity]
Given a finite set $V$, a function $f:2^V\mapsto \mathbb{R}$ is submodular if, for any subsets $S,T \subseteq V$, 
\begin{equation}
f(S) + f(T) \geq f(S\cap T) + f(S\cup T).
\end{equation}
$f$ is supermodular if $-f$ is submodular.
\end{mydef}

An equivalent definition is the following \cite{fujishige2005submodular}. 
A set function is submodular if, for any sets $S \subseteq T\subseteq V$ and any $v\in V\setminus T$, 
\begin{equation}
f(S \cup \{v\}) - f(S) \geq f(T \cup \{v\}) - f(T). \label{eq:equivalent_subomdular_def}
\end{equation}

Another useful property is \textit{monotonicity},  defined as follows. 

\begin{mydef}[Monotonicity]
Given a finite set $V$, a function $f: 2^V \mapsto \mathcal{R}$ is monotonic (or monotone) if, for any set $S\subseteq V$ and any $v\in V\setminus S$, $f(S \cup \{v\}) \geq f(S)$. 
\end{mydef}


If a set function $f(S)$ is submodular (and monotone), we can develop efficient algorithms for the following constrained optimization problems,
\begin{align}
\max\{f(S): S\in \mathcal{I}(\mathcal{M})\} \text{ and }\max\{f(S): S\in \mathcal{B}(\mathcal{M})\}.
\end{align}
where $\mathcal{I}(\mathcal{M})$ is the set of \textit{independent sets} and $\mathcal{B}(\mathcal{M}) \subseteq \mathcal{I}(\mathcal{M})$ is the set of bases of a \textit{matroid} $\mathcal{M}$, defined as follows.

\begin{mydef}[Matroid]
Let $V$ be a finite set, and let $\mathcal{I}$ be a collection of subsets of $V$. 
A set system $\mathcal{M}=(V, \mathcal{I})$ is a matroid if the following three conditions hold: (i) $\emptyset \in \mathcal{I}$, (ii) if $B \in \mathcal{I}$, then $A \in \mathcal{I}$ for all $A \subseteq B$, and (iii) if $A,B\in \mathcal{I}$ and $|A|<|B|$, then there exists $v \in B\setminus A$ such that $(A \cup \{v\}) \in \mathcal{I}$.
\end{mydef}

%The collection $\mathcal{I}$ is referred to as the set of \textit{independent sets} of the matroid $\mathcal{M}$. 
Each maximal independent set is a \textit{basis}. 
It can be shown that all bases of a matroid have the same size. 
The following lemma describes a property of submodular functions over matroid bases. 

\begin{mylemma}[\hspace{1sp}\cite{lee2010maximizing}]
Let $\mathcal{M}=(V,\mathcal{I})$ be a matroid, and let $f:2^V \mapsto \mathbb{R}$ be a submodular function defined on $V$. 
Let $S$ be a matroid basis such that, for all $u$ and $v$ with $u\in S$, $v\notin S$ and $(S \setminus \{u\} \cup \{v\}) \in \mathcal{I}$, $(1+\epsilon) f(S) \geq f(S \setminus \{u\} \cup \{v\})$. 
Then for any basic $C$ of $\mathcal{M}$, 
\begin{equation}
2(1+\epsilon) f(S) \geq f(S\cup C) + f(S \cap C).
\end{equation}
\end{mylemma}

The following lemma defines a sub-class of matroids called \textit{partition matroids}. 

\begin{mylemma}[Partition Matroid]\label{lemma:partition_matroid}
Let $V$ be a finite set, and $V_1$, ..., $V_m$ be a partition of $V$, that is, a collection of sets such that $V_1 \cup ... V_m=V$ and $V_i\cap V_j = \emptyset$ for $i\neq j$. 
Let $k_1$, ..., $k_m$ be a collection of nonnegative integers. 
Define a set $\mathcal{I}$ by $A \in \mathcal{I}$ iff $|A \cap V_i| \leq k_i$ for all $i=1,...,m$. 
Then $\mathcal{M}=(V, \mathcal{I})$ is a matroid, called a partition matroid. 
\end{mylemma}


==> ArXiv Submission/sections/proposed_algo.tex <==
\section{Proposed Algorithms}\label{sec:algo}
In this section, we first present our super-node formation algorithm that identifies %valid 
super-nodes 
%for a given channel 
and then present a greedy algorithm for max-cardinality and max-reward CA. 
Finally, we propose a local-search-based algorithm for max-utility CA, which exploits the structural property %called submodularity 
of the utility function and provides a performance guarantee. 

\subsection{Super-Node Formation}\label{sec:super_node_formation}
%As mentioned in Section~\ref{sec:conflict_graph_binary}, 
The super-node formation algorithm (Algorithm~\ref{algo:super_node_formation}) aims to identify a set of %super-nodes for a given channel $C$, i.e., 
nodes that have channel $C$ available and that are within each other's CS/ED range.
%As shown in Algorithm~\ref{algo:super_node_formation}, 
As we can see, 
the main input is an undirected graph, where each vertex is a node with $C$ available, and each edge \rev{connects two} nodes \rev{that} are within each other's CS/ED range. 
\rev{Since} a super-node is a \textit{clique} (a subgraph where every two distinct vertices are connected),  %on the graph, 
the first task is to find all such cliques.
In this work, we adopt the well-known Bron-Kerbosch algorithm \cite{bron1973algorithm},  a recursive backtracking algorithm that lists subsets of vertices that are cliques, and no listed subset can have any additional vertex without breaking its complete connectivity.
While a node can belong to multiple cliques, it randomly chooses a clique to join, since it cannot join two super-nodes at the same time.


\begin{algorithm}
\caption{Super-Node Formation}
\label{algo:super_node_formation}
\begin{algorithmic} [1]
\REQUIRE CS graph on channel $C$, activity index limit $\bar{\alpha}$
\ENSURE A set of super-NC pairs $U$ on channel $C$
\STATE Run Bron-Kerbosch algorithm to find cliques $\mathcal{Q}$.
\STATE	Each node in $V$ that belongs to multiple cliques chooses one to join (e.g., randomly).
\FORALL{clique $Q$ in $\mathcal{Q}$}
	\STATE	Run FFD to identify super-nodes $\mathcal{S}$ w.r.t. $\bar{\alpha}$.
	\STATE Add $(S,C)$ for each $S\in \mathcal{S}$ s.t. $|S|>1$ to $U$.
\ENDFOR
\RETURN $U$
\end{algorithmic}
\end{algorithm}
\normalsize

Although nodes in each clique (and any of its subsets) are able to coexist, the SAS may want to divide them into smaller groups for load balancing. 
Denote the \textit{activity index} of node $i$ as $\alpha_i > 0$, which is the estimated total number of channels it demands.
The activity index mapped to $C$ is $\alpha_i(C) = \min \left( \alpha_i/|C|, 1 \right) \in (0,1]$.
To avoid overcrowded super-nodes, the SAS can set a \textit{sum activity index limit} $\bar{\alpha}>0$ (e.g., $\bar{\alpha}=1.0$) for each super node. 
As a result, the task of grouping nodes (i.e., items with weights) into fewer super-radios (i.e., bins with capacity of $\bar{\alpha}$) becomes the well-known one dimensional \textit{bin packing problem} (BPP). 
In this work, we adopt a heuristic-based algorithm called \textit{first fit decreasing} (FFD)\cite{eilon1971loading}: it first creates a sequence of super-nodes (i.e., empty bins) and sorts nodes in non-increasing order of activity index; 
then it places each node into the lowest-indexed super-node with sufficient remaining space. 
Latest analysis has shown that FFD uses no more than $11/9$  OPT + $6/9$ bins, where OPT is the number of bins given by the optimal solution \cite{dosa2007tight}. 

\subsection{Algorithm for Max-Cardinality and Max-Reward CA}
\revv{In the max-cardinality CA (Eq.~(\ref{eq:max_cardinality_CA})), each vertex has a unit weight, while in the max-reward CA (Eq.~(\ref{eq:max_reward_CA})), each vertex has a weight equal to $(R(v)+\lambda |S(v)|)$. 
If we assume that each node has only one channel assignment, then the problems boil down to selecting an \textit{independent set} (IS), i.e., a set of vertices without any edges, that have the maximum sum of weights on general graphs, which is the classic \textit{maximum (weighted) independent set} (M(W)IS) problem.}
%Our proposed graph representation enables us to map the max-cardinality CA in Eq.~(\ref{eq:max_cardinality_CA}) to the classic \textit{maximum independent set} (MIS) problem, and the max-reward CA in Eq.~(\ref{eq:max_reward_CA}) to the generalized \textit{maximum weighted independent set} (MWIS) problem.
%Formally, given a vertex-weighted graph $G(V,E,R)$, a subset $I \subseteq V$ is an \textit{independent set} (IS) if for any two vertices $u,v\in I$, it holds that $e(u,v)\notin E$. The weight of a set $I$ is $R(I)=\sum_{v \in I} R(v)$, and an IS $I$ is maximum if there is no IS $I' \neq I$  such that $R(I) < R(I')$. 
%Since M(W)IS is NP-hard \cite{halldorsson2000approximations}, heuristic-based algorithms like GMWIS (Algorithm~\ref{algo:GWMIS}) are often used to obtain an approximate solution.
%\footnote{Apart from GMWIS, there exist other algorithms for MWIS. For example, authors in \cite{kako2005approximation} defined a metric called the weighted average degree and proposed greedy algorithms with provable performance.  Randomized algorithms like Tabu search \cite{hertz1987using} may also provide good results for MWIS. In this study, we adopt GMWIS due to its simplicity and low computational complexity, but more sophisticated MWIS algorithms may be implemented in practice.}.
%Denote by $\theta(G)$ the weight of a maximum IS, and by $A(G)$ the weight of the solution obtained by algorithm $A$.
%The performance ratio is defined by $\rho_A = \inf_G \frac{A(G)}{\theta(G)}$.
%GMWIS in Algorithm~\ref{algo:GWMIS} has the following performance guarantee. 
%It has been shown in \cite{sakai2003note} that GMWIS outputs an IS of weight at least $\sum_{v\in V} \frac{R(v)}{\delta_G(v)+1}$, where $\delta_G(v)$ is the vertex degree of $v$ and its performance ratio is $\frac{1}{\Delta_G}$, where $\Delta_G$ is the maximum vertex degree of $G$.
%Note that the computational complexity of Algorithm~\ref{algo:GWMIS} is $O(|V|^2)$, since each iteration takes $O(|V|)$ operations and there are up to $|V|$ iterations.

\revv{Since it is well known that both MIS and MWIS are NP-hard on general graphs\footnote{It has been shown that the problem may become easy on simple classes of graphs. For instance, MWIS can be solved in linear time in any tree graph. Polynomial time algorithms exist for MWIS in other classes of graphs including bipartite graphs, line graphs, circle graphs, claw-free graphs and planar graphs. See \cite{bandyapadhyay2014variant} for a brief summary.} \cite{halldorsson2000approximations,hastad1996clique}, it means that our problems are also NP-hard even when each node has only one channel assignment.} 
In this work, we adopt a heuristic-based algorithm %\footnote{Apart from GMWIS, there exist other algorithms for MWIS. For example, authors in \cite{kako2005approximation} defined a metric called the weighted average degree and proposed greedy algorithms with provable performance.  Randomized algorithms like Tabu search \cite{hertz1987using} may also provide good results for MWIS. In this study, we adopt GMWIS due to its simplicity and low computational complexity, but more sophisticated MWIS algorithms may be implemented in practice.} 
called GMWIS (Algorithm~\ref{algo:GWMIS}) to obtain an approximate solution.
Denote by $\theta(G)$ the weight of a maximum IS, and by $A(G)$ the weight of the solution obtained by algorithm $A$.
The performance ratio is defined by $\rho_A = \inf_G \frac{A(G)}{\theta(G)}$.
%GMWIS in Algorithm~\ref{algo:GWMIS} has the following performance guarantee. 
It has been shown in \cite{sakai2003note} that GMWIS outputs an IS of weight at least $\sum_{v\in V} \frac{R(v)}{\delta_G(v)+1}$, where $\delta_G(v)$ is the vertex degree of $v$ and its performance ratio is $\frac{1}{\Delta_G}$, where $\Delta_G$ is the maximum vertex degree of $G$.
Note that the computational complexity of Algorithm~\ref{algo:GWMIS} is $O(|V|^2)$, since each iteration takes $O(|V|)$ operations and there are up to $|V|$ iterations.

%\begin{mytheorem}[\hspace{0.01cm}\cite{sakai2003note}]\label{theorem:MWIS}
%GMWIS outputs an independent set of weight at least $\sum_{v\in V} \frac{R(v)}{\delta_G(v)+1}$ with a performance ratio of $1/\Delta_G$, where $\Delta_G$ is the maximum vertex degree of graph $G$.
%\end{mytheorem}

\begin{algorithm}
\caption{Greedy algortihm for MWIS (GMWIS)}
\label{algo:GWMIS}
\begin{algorithmic} [1]
\REQUIRE Vertex-weighted undirected graph $G(V, E, R)$
\ENSURE A maximal independent set $I$ in $G$

\STATE Pick a vertex $v\in V$ that maximizes $\frac{R(v)}{\delta_{G}(v) + 1}$. %, where $R(v)$ is the weight and $\delta_G (v)$ is the vertex degree in $G$\;
\STATE Add $v$ to $I$ and remove $v$ and its neighbors from $V$.
\STATE Repeat steps 1 and 2 until all vertices in $V$ are removed.	
\RETURN $I$

\end{algorithmic}
\end{algorithm}


%\subsection{Two-Phase Algorithm for Min-Demand-Max-Reward CA}
%One issue with max-reward CA and GMWIS is that they do not explicitly consider the min-demand constraint in the original formulation in Eq.~(\ref{eq:GAA_CA_formulation}).
%It means that the SAS may assign a large number of channels to a small subset of nodes, while others do not receive any channel. 
%Therefore, it makes more sense for the SAS to first meet the minimum demand of as many nodes as possible with best efforts, and then maximize the total reward. 
%
%To this end, we propose a two-stage algorithm based on GMWIS. 
%The main challenge is that due to channel contiguity, NC pairs available in Phase-II heavily depend on Phase-I selections.
%Hence, the SAS should reserve as many extensions as possible for Phase II in Phase I. 
%Details of our two-phase min-/max-demand CA are as follows.
%
%\subsubsection{Phase I -- Min-Demand CA}
%Denote the set of NC pairs for node $i$ as $V_i$, and the set of min-demand pairs as $V_i'$. 
%The SAS is interested in min-demand NC pairs $V'=\bigcup_{i}V_i'$ and the induced  subgraph $G[V']$.
%%\footnote{Our min-demand CA algorithm can handle arbitrary minimum demands, and radios with zero minimum demand will be temporarily ignored in this phase. From practical considerations, it is desirable to make the minimum demand be one or two channels, since GAA radios are unlicensed users after all and SAS allocates channels with best efforts;
%%otherwise, greedy GAA radios can aggressively ask for a large number of channels, which makes CA very difficult for SAS. 
%%} 
%Since it is equally important to meet any node's minimum demand, we adopt the cardinality-based weighting function $R(S,C)=|S|$.
%Then the problem becomes an instance of MWIS:  
%selecting a subset $I'\subseteq V'$ that maximizes $R(I')$ subject to the conflict-free constraint.
%%Denote the optimal solution as $I'_{OPT}$, and we know that  $|W(I'_{OPT})|=|U|$ due to the one-channel-assignment-per-radio constraint. 
%
%\begin{algorithm}
%\caption{Conflict-Free Min-demand CA}
%\label{algo:min_demand_CA}
%\begin{algorithmic} [1]
%\REQUIRE Conflict graph $G=(V,E)$
%\ENSURE An independent set of min-demand NC pairs $I'$
%
%\STATE Let 	$V'_i$ be the set of min-demand RC pairs for each node $i$, and $V'=\cup_{i} V'_i$\; 
%\STATE For each vertex $v=(S,C) \in V'$, let $R(v)=|S|$\;
%\STATE Pick a vertex $v \in V'$ that maximizes $\frac{R(v)}{\delta_{G[V']}(v) + 1}$\;
%\STATE To break ties, pick the one that minimizes $\delta_{G[V_{-S} \cup \{v\}]}(v)$, and maximizes the number of successors\;
%\STATE Add $v$ to the solution $I'$\;
%\STATE Remove $v$ and its neighbors in $V'$ from $V'$\;
%\STATE Remove $v$ and its neighbors except its successors in $V$ from $V$\;
%\STATE Repeat steps 3 through 7 until all vertices in $V'$ are removed from the graph\;		
%
%\end{algorithmic}
%\end{algorithm}
%
%Our min-demand CA algorithm is described in Algorithm~\ref{algo:min_demand_CA}.
%It greedily selects the next best vertex that maximizes $\frac{R(v)}{\delta_{G[V']}(v) + 1}$ as in GMWIS. 
%Note that $\delta_{G[V']}(v)$ for $v=(S,C)$ is the  count of i) alternative min-demand NC pairs for nodes in $S$, and ii) min-demand NC pairs at conflicted nodes that would become unavailable, if $v$ is selected. 
%Hence, the above criterion gives higher priority to nodes that have fewer available channels and are more ``friendly'' to others.
%
%In the presence of ties, heuristics are used to break them (Line 4) instead of random selection, and the one with fewer \textit{inter-node conflicts} is chosen. 
%Let the set of \textit{all} NC pairs (including non-min-demand ones) for nodes other than $S$ be  $V_{-S}=V\setminus (\bigcup_{i\in S}V_i)$. 
%The number of inter-node conflicts of $v$ on $G$ is $\delta_{G[V_{-S} \cup \{v\}]}(v)$, which is the number of NC pairs at other nodes that would become unavailable due to $v$.
%In summary, it is preferred to select NC pairs that are more ``friendly'' to other nodes. 
%
%If a tie further exists, the one with more  ``successors'' is chosen. 
%Formally, given two NC pairs $v_1=(S_1, C_1)$ and $v_2=(S_2, C_2)$, $v_2$ is considered a successor of $v_1$, if $S_1 \subseteq S_2$ and $C_1 \subset C_2$.
%In other words, it is possible for the SAS to assign more channels $C_2 \setminus C_1 \neq \emptyset$ to nodes in $S_1$ after selecting $v_1$ without violating channel contiguity.
%A further tie will be broken randomly.
%Intuitively, the above heuristics are meant to reserve more valid NC pairs for Phase II. 

%After $v$ is selected, $v$ and its neighbors in $V'$ are removed from $V'$.
%$v$ and its neighbors in $V$ from $V$, but its successors are kept.
%This is because we want to avoid eliminating possible Phase-II extensions of our current selection, when selecting subsequent min-demand pairs.

%\subsubsection{Phase II -- Max-Reward CA}
%Given the Phase-I output $I'$, the SAS determines the set of NC pairs in $V\setminus I'$ that are successors of $I'$, denoted as $\tilde{V}$. 
%The objective of the SAS is to select an IS $\tilde{I} \in \tilde{V}$ that maximizes the total reward $R(\tilde{I})$, which is once again an instance of MWIS, and Algorithm~\ref{algo:GWMIS} is in place to provide an approximate solution. 
%After $\tilde{I}$ is obtained, NC pairs in $I'$ that conflict with any NC pair $v$ in $\tilde{I}$ (i.e., predecessors of $v$) become invalid due to the one-channel-assignment-per-node constraint. 
%Hence, the final output is given by $I=\tilde{I} \cup \{v: v\in I', e(v,u)\notin E, \forall u\in \tilde{I} \}$.
\vspace{-0.3cm}

\subsection{Proposed Algorithm for Max-Utility CA}
In this section, we first provide brief background on submodularity and matroids. 
Then we show that the max-utility CA problem in Eq.~(\ref{eq:max_utility_CA}) is matroid-constrained submodular maximization and proposed a polynomial-time algorithm with a provable performance guarantee.

\subsubsection{Background on Submodularity and Matroids}
Submodularity is a property of set functions that captures the \textit{diminishing returns} behavior, that is, adding a new element introduces greater incremental benefits, if there are fewer elements so far, and less, if there are more elements.
  
The formal definition is as follows.

\begin{mydef}[Submodularity]
Given a finite set $V$, a function $f:2^V\mapsto \mathbb{R}$ is submodular if, for any subsets $S,T \subseteq V$, 
\begin{equation*}
f(S) + f(T) \geq f(S\cap T) + f(S\cup T).
\end{equation*}
%$f$ is supermodular if $-f$ is submodular.
\end{mydef}

An equivalent definition is the following \cite{fujishige2005submodular}. 
A set function is submodular if, for any sets $S \subseteq T\subseteq V$ and any $v\in V\setminus T$, 
\begin{equation}
f(S \cup \{v\}) - f(S) \geq f(T \cup \{v\}) - f(T). \label{eq:equivalent_subomdular_def}
\end{equation}

%\begin{mydef}[Submodularity \cite{fujishige2005submodular}]\label{def:submodularity}
%Given a finite set $V$, a function $f:2^V\mapsto \mathbb{R}$ is submodular if, for any sets $S \subseteq T\subseteq V$ and any $v\in V\setminus T$, 
%\begin{equation*}
%f(S \cup \{v\}) - f(S) \geq f(T \cup \{v\}) - f(T). \label{eq:equivalent_subomdular_def}
%\end{equation*}
%\end{mydef}

%Another useful property is \textit{monotonicity},  defined as follows. 
%
%\begin{mydef}[Monotonicity]
%Given a finite set $V$, a function $f: 2^V \mapsto \mathcal{R}$ is monotonic (or monotone) if, for any set $S\subseteq V$ and any $v\in V\setminus S$, $f(S \cup \{v\}) \geq f(S)$. 
%\end{mydef}

%Another important concept is \textit{matroid}, defined as follows.

\begin{mydef}[Matroid]\label{def:matroid}
Let $V$ be a finite set, and let $\mathcal{I}$ be a collection of subsets of $V$. 
A set system $\mathcal{M}=(V, \mathcal{I})$ is a matroid if the following three conditions hold: (i) $\emptyset \in \mathcal{I}$, (ii) if $B \in \mathcal{I}$, then $A \in \mathcal{I}$ for all $A \subseteq B$, and (iii) if $A,B\in \mathcal{I}$ and $|A|<|B|$, then there exists $v \in B\setminus A$ such that $(A \cup \{v\}) \in \mathcal{I}$.
\end{mydef}

%Each maximal independent set is a \textit{basis}. 
%It can be shown that all bases of a matroid have the same size. 
%The following lemma describes a property of submodular functions over matroid bases. 

Given a matroid $\mathcal{M}$, $\mathcal{I}(\mathcal{M})$ is called the set of \textit{independent sets} of $\mathcal{M}$.
A sub-class of matroids called \textit{partition matroids} is defined as follows.

\begin{mydef}[Partition Matroid]\label{def:partition_matroid}
Let $V$ be a finite set, and $V_1$, ..., $V_m$ be a partition of $V$, that is, a collection of sets such that $V_1 \cup ... V_m=V$ and $V_i\cap V_j = \emptyset$ for $i\neq j$. 
Let $k_1$, ..., $k_m$ be a collection of nonnegative integers. 
Define a set $\mathcal{I}$ by $A \in \mathcal{I}$ iff $|A \cap V_i| \leq k_i$ for all $i=1,...,m$. 
Then $\mathcal{M}=(V, \mathcal{I})$ is a matroid, called a partition matroid. 
\end{mydef}

\subsubsection{Matroid-Constrained Submodular Maximization}
As we can see, the constraint in the max-utility CA formulation in Eq.~(\ref{eq:max_utility_CA}) defines a partition matroid,
\begin{align}
\mathcal{M}=(V,~\mathcal{I}), \text{ where } \mathcal{I}&=\{I: |I \cap V_i| \leq 1, \forall i=1,2,...,n\} \nonumber \\
&\text{ and } \{V_i\} \text{ is a partition of } V, \label{eq:matroid_constraint}
\end{align}
and \rev{we can show that} the utility function in Eq.~(\ref{eq:utility_function}) is a submodular set function.  

\begin{mylemma}\label{lemma:submodular}
The utility function $U(\cdot)$ in Eq.~(\ref{eq:utility_function}) is submodular.  
\end{mylemma}
\begin{proof}
See Appendix~\ref{proof:lemma:submodular} for proof.
\end{proof} 

Hence, the problem $
\max\{U(I): I \in \mathcal{I}(\mathcal{M}) \}$ is an instance of matroid-constrained submodular maximization, \revv{which is known to be an NP-hard optimization problem \cite{lee2010maximizing}}.
%where $\mathcal{M}$ is the partition matroid defined in Eq.~(\ref{eq:matroid_constraint}).


\begin{algorithm}
\caption{Utility Maximization ({\tt UM})}
\label{algo:UM_algorithm}
\begin{algorithmic} [1]
\REQUIRE Partition matroid $\mathcal{M}=(V, \mathcal{I})$, utility function $U(\cdot)$, and parameter $\epsilon > 0$
\ENSURE $I$ -- Selected NC pairs

\STATE $I_1 \leftarrow$ {\tt LS} ($\mathcal{M}, U, \epsilon$)
\STATE $\mathcal{I}' \leftarrow \{I: |I \cap V'_i| \leq 1\}, \text{ where } V'_i = V_i \setminus I_1, \forall i = 1,2,...,n$
\STATE Define $\mathcal{M}'=(V', \mathcal{I}')$, where $V'=\cup_i V'_i$
\STATE $I_2 \leftarrow $ {\tt LS} ($\mathcal{M}', U, \epsilon$)
\RETURN $ I \leftarrow \arg\max_{I\in \{I_1, I_2\}} U(I)$

%\end{algorithmic}

\algrule
\vspace{-0.1cm}
\textbf{Local Search Procedure} ({\tt LS}):
\vspace{-0.1cm}
\algrule

%\begin{algorithmic} [1]
\REQUIRE Matroid $\mathcal{M}=(V, \mathcal{I})$, submodular function $f(\cdot)$, and parameter $\epsilon \geq 0$
\ENSURE A selected subset $I$

\STATE $I\leftarrow \emptyset$, $v \leftarrow \arg\max \{f(u)| u \in V\}$, $N \leftarrow |V|$. \label{algo:line:start}
\WHILE{$v\neq \emptyset$ and $f(I \cup \{u\}) > (1 + \frac{\epsilon}{N^2}) f(I)$}
	\STATE $I \leftarrow I \cup \{v\}$
	\STATE $v \leftarrow \arg\max \{f(I \cup \{u\}) - f(I) | u \in V\setminus I \text{ and } I \cup \{u\} \in \mathcal{I} \}$
\ENDWHILE \label{algo:line:end_of_greedy}

\WHILE{$true$}
	\IFTHEN {there exists $d \in I$ such that $f(I \setminus \{d\}) \geq (1+\frac{\epsilon}{N^2}) f(I)$} {$I \leftarrow I \setminus \{d\}$, \textbf{continue}} \label{algo:line:delete}
	\IFTHEN {there exists $a \in V \setminus I$ and $d \in I \cup \emptyset$ such that $I \setminus \{d\} \cup \{a\} \in \mathcal{I}$ and $f(I \setminus \{d\} \cup \{a\}) \geq (1 + \frac{\epsilon}{N^2}) f(I)$}
	{$I \leftarrow I \setminus \{d\} \cup \{a\}$, \textbf{continue}} \label{algo:line:add_swap}
	\STATE \textbf{break} 
\ENDWHILE
\RETURN $I$ \label{algo:line:end}
	
\end{algorithmic}
\end{algorithm}


\subsubsection{Proposed Algorithm}
Our algorithm {\tt UM} (Algorithm~\ref{algo:UM_algorithm}) is based on the (approximate) local search procedure {\tt LS} (Lines~\ref{algo:line:start}-\ref{algo:line:end}).
It \rev{quickly} finds an initial solution %with a single element (Line~\ref{algo:line:start}) and 
\rev{by iteratively adding the next element with the maximum incremental utility} (Lines~\ref{algo:line:start}-\ref{algo:line:end_of_greedy}) and then searches for the locally optimal solution under the local delete (Line~\ref{algo:line:delete}), add and swap (Line~\ref{algo:line:add_swap}) operations subject to the matroid constraint.
%Note that the initial solution is not limited to a single element, and can be a greedy or random solution as well.
To achieve faster convergence, the parameter $\epsilon$ can be set to obtain an approximately locally optimal solution.
Note that {\tt LS} is called twice in {\tt UM}: it first obtains $I_1$ for the original matroid $\mathcal{M}$ and then $I_2$ for the new matroid $\mathcal{M}'$, which corresponds to the partition $\{V_i'\}$ of $V'$ (i.e., $V \setminus I_1$). 
The set, either $I_1$ or $I_2$, that yields a greater utility is returned. 

Theorem \ref{theorem:bound} shows that {\tt UM} (Algorithm~\ref{algo:UM_algorithm}) provides a performance guarantee. 

\begin{mytheorem}\label{theorem:bound}
Algorithm~\ref{algo:UM_algorithm} returns a solution $I$ with the following performance guarantee
\begin{equation}
U(I) \geq \frac{1}{(4+2\epsilon)} [ U(OPT) + 2 U_{\min}],
\end{equation}
where $OPT$ is the optimal solution to $\max\{U(I): I \in \mathcal{I}(\mathcal{M})\}$, and $U_{\min} = \min \{U(I): I \in \mathcal{I}(\mathcal{M})\}$. 
If $U(\cdot)$ is non-negative (i.e., $U_{\min} \geq 0$), we have $U(I)\geq \frac{1}{(4+2\epsilon)} U(OPT)$.
\end{mytheorem}
\begin{proof}
See Appendix~\ref{proof:theorem:bound} for proof. 
\end{proof}

\begin{myproposition}\label{proposition:complexity}
Algorithm~\ref{algo:UM_algorithm} is in polynomial time with runtime bounded by $O(\frac{1}{\epsilon} N^3 \log N)$. 
\end{myproposition}
\begin{proof}
See Appendix~\ref{proof:proposition:complexity} for proof. 
\end{proof}

==> ArXiv Submission/sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}
Dynamic CA has been studied in different contexts including cellular networks \cite{katzela1996channel}, mesh networks \cite{si2010overview} and cognitive radio networks \cite{akyildiz2006next}.
Among the proposed approaches, \rev{graphs are widely adopted for CA modeling.}
%graph-based representations have been widely adopted. 
In \cite{cao2005distributed, wang2005list, peng2006utilization,hessar2014resource}, authors considered CA \rev{under the} channel availability and interference constraints \rev{using} vertex-weighted interference/conflict graphs, where each vertex represents a user with a color \rev{(channel)} list, and each edge denotes a binary conflict due to co-channel interference.
The problem is then formulated as graph multi-coloring (i.e., assign %multiple 
conflict-free colors to users and obtain rewards on vertices) and a typical objective is to maximize the total reward or utility (derived from rewards).
Such conflict-free CA algorithms %channel assignments 
are suitable for sparse networks with QoS consideration for each user.

In order to capture the interference with greater granularity, non-binary conflicts using an edge-weighting or penalty function may be introduced, and typical objectives include minimizing the total interference or penalty via graph coloring \cite{mishra2005weighted, subramanian2007fast, yue2011cacao} or maximizing the total reward subject to the aggregate interference limit at each user \cite{hoefer2014approximation,hessar2014resource}. 
However, \rev{the vast majority} of existing works do \textit{not} consider geographic and channel contiguity constraints \rev{and thus are} not applicable to CA in the CBRS. 
In \cite{subramanian2008near}, Subramanian \textit{et. al.} introduced the notion of channel graph to enforce channel contiguity,  %(in addition to the interference graph), 
where each vertex is a channel consisting of several contiguous primitive channels and each edge \rev{indicates overlapping channels.}
%\rev{But their proposed graphs do not account for location-dependent channel contiguity. 
\rev{In Section~\ref{sec:evaluation_max_reward_CA}, we will show that our proposed algorithm outperforms the algorithm in \cite{subramanian2008near} in terms of accommodating more users and meeting greater demand. 
}

%But they assumed the same channel graph at each user without considering channel availability, and the proposed approach only provides a conflict-free solution, which implies that many GAA devices may not receive a channel in a dense network. 

\begin{figure*}[!ht]
	\centering
	\subfloat[]{\includegraphics[width=1\columnwidth]{./figs/channel_assignment_example}\label{fig:channel_assignment_example1}}
	\subfloat[]{\includegraphics[width=.8\columnwidth]{./figs/channel_assignment_example2}\label{fig:channel_assignment_example2}}
	\caption{Illustration of the PA CA scenario. 
		(a) A holds one PAL in its service area that consists of tracts 1 and 3, while B stacks two PALs in its service area that consists of tracts 1 and 2.  
		Each PA CBSD deployed by the licensee has a PPA that cannot extend beyond its service area. 
		GAA nodes may reuse assigned PAL channels at locations beyond the PPAs, subject to the interference constraint. 
		(b) Given three PAL channels, the SAS can assign CH $\{1\}$ in tracts $1$ and $3$ to A's PALs and CH $\{2,3\}$ in tracts $1$ and $2$ to B's PALs, so as to meet the geographic and channel contiguity requirements.
	}
	\label{fig:channel_assignment_example}
\end{figure*}

\rev{In this work, we incorporate the contiguity constraints by introducing (super)NC-pair conflict graphs, which can also be used to represent channel availability and enhance coexistence awareness. 
Besides, the proposed conflict graph allows us to relate the PA CA and binary GAA CA to the classic the maximum (weighted) independent set problem \cite{halldorsson2000approximations,sakai2003note,kako2005approximation} and adopt a widely used heuristic-based algorithm that runs in polynomial time with a performance guarantee.
To further enhance coexistence awareness, we consider non-binary GAA CA and formulate the problem as utility maximization.}
We then prove the submodularity of the utility function and
%, and show that it is an instance of matroid-constrained submodular maximization problem in combinatorial theory \cite{lee2010maximizing}.
propose a polynomial-time algorithm based on local search with a provable performance guarantee.
%\rev{To the best of our knowledge, this is the first work that exploits the submodularity property to develop a CA algorithm.}

%\rev{Our extensive simulations using a real-world dataset %Wi-Fi hotspot location dataset for a dense Wi-Fi network in NYC 
%	have demonstrated the advantages of the proposed graph representation and the superior performance of the proposed algorithms against baseline algorithms.}


%\noindent \textbf{Construction of conflict graphs:}
%\cite{zhou2013practical} discusses how to construct practical conflict graphs from measurements. 
%\cite{jain2005impact} proposed protocol and physical models to determine the interference relationship in a multi-hop wireless network.
%
%Measurement-based: In \cite{reis2006measurement} authors proposed practical models for the physical layer behaviors of packet reception and carrier sense with interference in static wireless
%networks. 
%These models use measurements (i.e., RSSI values) of a real network rather than abstract RF propagation models as the basis for accuracy in complex environments.
%One application was to estimate the conflict graph used in \cite{jain2005impact}.
%
%In \cite{qiu2007general}, authors develop a general model to estimate the throughput and goodput between arbitrary pairs of nodes in the presence of interference from other nodes in a wireless network. 
%Our model is based on measurements from the underlying network itself and is thus more accurate than abstract models of RF propagation such as those based on distance.




==> ArXiv Submission/sections/sas_assisted_channel_assignment.tex <==
\section{Channel Assignment \rev{in CBRS}}\label{sec:channel_assignment_scenario}
In this section, we describe CA scenarios for PA and GAA tiers based on the FCC rules \cite{fcc2012, fcc2014, fcc2015, fcc2016}.
In particular, we highlight CA challenges and opportunities in the CBRS: geographic and channel contiguity, spatially varying channel availability, flexible demands, and coexistence awareness. 
\rev{Then we present the architecture of SAS from the perspective of dynamic CA. }

%\subsection{Architecture of CBRS and SAS}
%\res{As illustrated in Fig.~\ref{fig:CBRS_architecture}, three types of CBSD networks are envisioned in \cite{kim2015design}: 1) A traditional cellular operator deploying small cells that combine traditional licensed bands with the 3.5 GHz band, 2) A cable Wi-Fi operator or fiber-to-home operators that combine traditional Wi-Fi bands with the 3.5 GHz band, and 3) indoor operator networks deployed in large enterprises or places like hospitals etc. that offer indoor wireless access in the 3.5 GHz band.}
%
%\begin{figure}[!t]
%	\centering
%	\subfloat[]{\includegraphics[width=.55\columnwidth]{./figs/CBRS_architecture}\label{fig:CBRS_architecture}}
%	\subfloat[]{\includegraphics[trim=0 -2cm 0 0,clip=true,width=.43\columnwidth]{./figs/SAS_functional_architecture2}\label{fig:SAS_functional_architecture2}}
%	\caption{(a) System architecture of the CBRS. % (adapted from \cite{kim2015design}). 
%	(b) Functional architecture of the SAS. 
%	% \cite{winnforum2018requirements}. %sohul2015spectrum
%	}
%	\label{fig:SAS_architecture}
%\end{figure}
%
%\res{Fig.~\ref{fig:SAS_functional_architecture2} illustrates the architecture of the SAS as a centralized entity that manages CBSDs \cite{winnforum2018requirements}. 
%The signaling protocol between the SAS and CBSDs enables procedures such as (de)registration, spectrum inquiry, grant (relinquishment), and heatbeat \cite{winnforum2018signaling}. 
%Every CBSD is required to register with the SAS and provide information such as location and installation parameters (e.g., antenna height and gain). 
%Based on CBSD information and incumbent activities, the SAS will determine available channels and performs CA for PA users, followed by GAA CA. 
%As a matter of fact, centralized CA algorithms are well suited for the SAS as part of the PA and GAA managers.}

%The reference architecture of the SAS is defined by the WInnForum \cite{winnforum2017requirements} and illustrated in Fig.~\ref{fig:SAS_functional_architecture}.
%The main component is SAS 1 that authorizes and manages use of spectrum for CBRS. 
%Specifically, it determines available channels and assigns them to different CBSDs, and determines the maximum permissible power levels for CBSDs at their locations.
%It also enforces interference protection for incumbents and PA users.
%
%As we can see, SAS 1 can communicate either directly with individual CBSDs, or indirectly via the domain proxy through the SAS-user interface. 
%It also communicates with other SAS's using messaging protocols via the SAS-SAS intrefrace.
%Each SAS is connected to FCC databases to retrieve latest information about FSS earth stations.
%To protect shipborne radars, the SAS exploits the information from Environment Sensing Capability (ESC) devices or CBSDs with sensing capability.
%
%\begin{figure}[ht!]
%	\centering
%	\includegraphics[width=.95\columnwidth]{./figs/SAS_functional_architecture}
%    \caption{SAS reference architecture.}
%    \label{fig:SAS_functional_architecture}
%\end{figure}
%
%The rules \cite{fcc2016} define two typse of CBSDs: 
%Category A devices similar to indoor/outdoor small cells, and Category B for point-to-point use. 
%The maximum EIRP for Category A and B CBSDs is 30 dBm and 47 dBm over a 10 MHz channel, respectively. 
%In this paper, we focus on channel assignment for Category A CBSDs, and also refer to a CBSD as an access point (AP) in the rest of this work. 

\subsection{PA CA Scenario}\label{sec:PA_channel_assignment}
%As per \rev{the} FCC rules \cite{fcc2016}, a 
%A PAL is defined as a short-term, non-renewable authorization to use a channel in a license area.
As per the FCC rules, %up to $7$ out of $10$ channels in the 3550-3650 MHz band can be reserved for PALs, and up to 4 channels can be aggregated by the same licensee in each license (or service) area.
%\subsubsection{License Area, Service Area and PAL Protection Area}\label{sec:scenario_PA_CA}
%\subsubsection{PAL Protection Area (PPA)}\label{sec:scenario_PA_CA}
%A \textit{License Area} is a census tract, and a \textit{Service Area} consists of one or more \textit{contiguous} license areas held by the same PA licensee.
each deployed PA CBSD has an associated PPA with a default protection contour that is calculated based on the signal level of $-96$ dBm/$10$ MHz, which cannot extend beyond the licensee's service area.
%that consists of one ore more contiguous license areas.
A self-reported PPA contour is also acceptable, so long as it is within the default PPA contour.
%Note that the PAA cannot extend beyond the licensee's license or service area. 
If PPAs for multiple CBSDs operated by the same licensee overlap, they would be merged into a single PPA. 
Note that interference protection is \rev{enforced} for each active PPA, that is, the aggregate co-channel interference from other PA or GAA CBSDs at any location within a PPA cannot exceed $-80$ dBm/$10$ MHz. %(measured with an antenna of height $1.5$ meters above ground). 
%Adjacent channel interference may not be considered by the SAS due to stringent out-of-channel emission limits.
%The above requirement does not apply to adjacent census tracts held by the same licensee. 

%To keep PPA active, CBSDs shall contact the SAS regularly. 
%; otherwise, the protection will be discontinued, if there is no contact within $7$ days.
%Also, CBSDs shall inform the SAS of any change in protection areas. 

%\subsubsection{Interference Protection}
%It is important to note that interference protection is enforced for each active PPA, not service area. 
%The aggregate co-channel interference from other PA or GAA CBSDs at locations within a PPA cannot exceed $-80$ dBm/$10$ MHz (measured with an antenna of height $1.5$ meters above ground). 
%Adjacent channel interference may not be considered by the SAS due to stringent out-of-channel emission limits.
%The above requirement would not apply to adjacent census tracts held by the same licensee. 

%\subsubsection{CA Requirements}
%According to %\textsection 96.25 in 
%\cite{fcc2015}, 
The FCC imposes two contiguity requirements for PA CA: 1) \textit{geographic contiguity} -- an SAS must assign geographically contiguous PALs held by the same PA licensee to the same channels in each geographic area, to the extent feasible; and 2) \textit{channel contiguity} -- an SAS must assign multiple channels held by the same PA licensee to contiguous channels in the same license area, to the extent feasible.
An example is provided in Fig.~\ref{fig:channel_assignment_example} that illustrates the PA CA scenario. %\footnote{\revv{It is worth noting that in cases where two adjacent, non-overlapping service areas are assigned the same channel, locations close to the service area boundaries may not be suitable for PA CBSD deployment. Suppose that two PA CBSDs operated by different licensees are deployed close to the boundary. When operating co-channel, the two CBSDs may cause interference that exceeds the -80 dBm/10 MHz interference limit to each other. While this issue may occur in practice, the SAS's objective for PA CA is to assign channels to PALs, and thus we do not consider addressing this issue as the SAS's responsibility.}}.

%\begin{itemize}
%\item \textit{Geographic contiguity}: An SAS must assign geographically contiguous PALs held by the same PA licensee to the same channels in each geographic area, to the extent feasible.
%
%\item \textit{Channel contiguity}: An SAS must assign multiple channels (up to $4$) held by the same PA licensee to contiguous channels in the same license area, to the extent feasible.
%\end{itemize}
%The SAS may temporarily reassign PALs to non-contiguous channels to protect incumbents.

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=.7\columnwidth]{./figs/channel_assignment_example}
%	\caption{ 
%	}
%	\label{fig:channel_assignment_example}
%\end{figure}


%\subsubsection{Example}\label{sec:PA_example}
%\rev{In order to illustrate the PA CA scenario, we provide an example} in Fig.~\ref{fig:channel_assignment_example}, in which A holds one PAL in the service area that consists of tracts 1 and 3, while B stacks two PALs in its service area that consists of tracts 1 and 2 (Fig.~\ref{fig:channel_assignment_example1}). 
%Since the two service areas are overlapping, exclusive channels must be assigned by the SAS.
%After channels are assigned to PALs, operators may deploy PA CBSDs that operate in the assigned channel(s) inside their respective service areas.
%Given three PAL channels, the SAS may assign CH $1$ to A's PALs in tracts 1 and 3, and CH $\{2,3\}$ to B's PALs in tracts 1 and 2 (Fig.~\ref{fig:channel_assignment_example2}) to meet the contiguity requirements. 


\subsection{GAA CA Scenario}
%Due to the hierarchical spectrum access framework, the SAS performs GAA CA after PA CA, and any significant changes in the PA tier may trigger channel re-assignment in the GAA tier.
%Besides, GAA CBSDs must provide the SAS with all information required by the rules, including operator/device ID, location, upon initial registration and as required by the SAS. 

%Moreover, GAA CBSDs access the spectrum on a shared and equitable basis, and should expect no interference protection. 
GAA CA \rev{differs} from PA CA in the following aspects. 
First, channel availability for GAA nodes can vary significantly depending on location.
This is because a PAL channel is considered ``in use'' only within PPAs and becomes available for GAA use at a location beyond the PPAs (and their vicinities), % under the ``use-it-or-share-it'' rule, 
if GAA transmission at that location does not cause 
\rev{over-the-limit interference} %interference higher than $-80$ dBm/$10$ MHz 
at any location within PPAs. 
%In practice, the set of available channels for a GAA CBSD may be determined by the SAS, based on information including location, RF parameters (e.g., transmit power and antenna gain), %\footnote{As per the FCC rules \cite{fcc2015}, GAA CBSDs must provide the SAS with all information required by the rules, including operator/device ID, location, upon initial registration and as required by the SAS. }, 
%the interference model and PPAs. %, which may vary significantly in space.  
As illustrated in the example in Fig.~\ref{fig:channel_assignment_example}, GAA nodes $G_1$ and $G_4$ are located in the service area of PA licensees, but they are free to use all channels just like $G_5$, since they do not cause significant interference to any PA CBSD. 
In contrast, $G_2$ cannot operate co-channel with $A_2$, and $G_3$ cannot operate co-channel with $B_3$, due to the interference constraint. 
Although it is not desirable for $G_2$ and $G_3$ to operate co-channel as they would interfere with each other, it is indeed acceptable as per the FCC ruling. 


%\subsubsection{Channel Availability}
%Channels assigned to PALs are considered ``in use'' only within PPAs, and those beyond PPAs are available for GAA use under the ``use-it-or-share-it'' rule. 
%As a result, channels that are available for a GAA CBSD depend on location, which may vary significantly in space. 
%As shown in Fig.~\ref{fig:channel_assignment_example}, there are 7 GAA CBSDs, labeled from $G_1$ to $G_7$.
%The dashed circle denotes the interference contour of a CBSD given its transmission power, which cannot  overlap with any co-channel PAL protection area.
%Given PA channel assignments in Section~\ref{sec:PA_example}, $G_2$ has two available channels (CH 2 and 3), while $G_7$ has only CH 1 available. 

Second, a GAA node may request multiple contiguous channels (up to a certain limit such as four), \rev{and the demand could be very flexible}. % along with the channel contiguity requirement. 
For instance, a Wi-Fi node may request two contiguous channels but would be very willing to receive four to obtain higher capacity.
Although the SAS is not obligated to meet the maximum demands of all GAA nodes, it \rev{would be expected to} maximize the number of assigned channels or the overall throughput with best efforts.

\begin{figure*}[h!]
	\centering
	\includegraphics[width=.7\textwidth]{./figs/SAS_assisted_CA_architecture}
	\caption{Architecture of SAS as a centralized entity from the perspective of dynamic CA. A centralized PA/GAA CA algorithm will be implemented in the PA/GAA manager within the SAS. Note that only data flows for PA/GAA CA purposes are highlighted.}
	\label{fig:SAS_assisted_CA_architecture}
\end{figure*}

%\subsubsection{Coexistence Awareness}
Third, GAA nodes are expected to coexist in the same frequency, space and time. 
In this work, we consider co-channel coexistence enabled by Wi-Fi like MAC protocols such as CSMA/CA in Wi-Fi \cite{80211ac2013} and Listen-Before-Talk in LAA \cite{etsi2016lte}. 
Traditional channel assignment techniques \cite{cao2005distributed, wang2005list, peng2006utilization} typically model interference as a binary conflict and avoid assigning the same channel to any two conflicting nodes.
However, two interfering nodes in close proximity are able to detect each other's transmission (i.e., no hidden nodes) and share the same channel(s) in the CSMA/CA fashion.  
Hence, the SAS may exploit such opportunities to accommodate more nodes in this case, especially when the spectrum is crowded. 
In this work, we further consider non-binary conflicts in terms of penalties to enhance \textit{coexistence awareness}. %More discussions are available in Section~\ref{sec:coexistence_awareness}.

%As shown in Fig.~\ref{fig:channel_assignment_example}, there are three possible cases for co-channel deployment of GAA CBSDs. 
%For simplicity, we assume the same communication, carrier-sensing and interference ranges.
%In the first case, two CBSDs (i.e., $G_1$ and $G_2$) are located far away from each other, and thus they may be assigned to the same channel without interference. 
%When two CBSDs get closer like $G_3$ and $G_4$, they are hidden from each other for downlink transmissions, and may cause interference to clients located in the overlapping region. 
%Hence, it is better to assign different channels to them if possible, or otherwise, they may incur additional signaling overhead associated with client feedback in order to resolve the hidden node problem. 
%
%In the third case, two CBSDs are close enough and within the carrier-sensing range of each other, like $G_5$ and $G_6$. 
%Thanks to Wi-Fi like protocols, they are able to coexist co-channel, and share channel access time or throughput. 
%Therefore, the SAS should be aware of such coexistence opportunities, which is referred to as \textit{coexistence awareness}. 

%To summarize, the SAS needs to consider spatial channel availability variation and enforce geographic/channel contiguity for PA and GAA channel assignments, as well as be aware of coexistence opportunities for GAA channel assignment.

\res{
\subsection{Architecture of SAS-Assisted Dynamic CA}
As shown in Fig.~\ref{fig:SAS_assisted_CA_architecture}, the SAS is a centralized entity consisting of incumbent, PA and GAA managers.
It communicates with the Environment Sensing Capability (ESC) component, FCC databases (DBs), and CBSDs. 
The PA manager receives information on DPAs and PALs, determines PAL channel availability based on the interference model and requirements, and executes the PA CA algorithm to assign channels to PALs grouped by service areas.  
The GAA manager takes as inputs 1) the PPAs and PA CA results, 2) GAA CBSD registration information (e.g., location, transmit power, and antenna gain), 3) CBSD demands and activity indices (i.e., traffic load indicators), and 4) the interference model\footnote{Radio propagation models, despite their limitations, are still widely used for initial network planning, but the interference relationship can also be determined from real measurements. Such measurement reporting is already supported by the WInnForum SAS-CBSD protocol \cite{winnforum2018signaling}.} and requirements. 
It then determines channel availability for GAA nodes and executes the GAA CA algorithm. 
Finally, the SAS will disseminate the PA and GAA CA results to individual CBSDs (e.g., within 10s of seconds). 

According to the WInnForum SAS-CBSD protocol specifications \cite{winnforum2018signaling}, the protocol exchange between the SAS and CBSDs already exists, including requests and responses for (de)registration, spectrum inquiry, grant (relinquishment) and heatbeat.
Therefore, the SAS can readily leverage registration and regular heartbeat messages to collect inputs from CBSDs and use them for CA purposes, without introducing additional signaling overhead. 

It is also important to note that the CA in the CBRS is indeed dynamic:  changes in DPAs and PALs would trigger PA CA, which further trigger GAA CA along with other factors (e.g., changes in GAA CBSD demands). 
Since DPA and PAL changes are relatively infrequent, PA channel assignments will be expected to be quasi-stable, and channel reassignment occurs presumably in the order of hours or days. In contrast, the SAS may have to aggregate demands from all GAA nodes and perform GAA CA periodically (e.g., every 100s of seconds).
Nevertheless, the SAS can always take a snapshot of the CBSD network at a given time instant and perform CA for PA and GAA tiers separately in a centralized fashion\footnote{The SAS itself may be implemented in a distributed cloud so as to exploit dedicated computing resources spread over multiple virtual machines to perform CA for a specific region.}. }




==> sections/preliminaries.tex <==
\section{Preliminaries}
In this section, we briefly review some concepts in graph theory and introduce notations that will be used throughput this paper. 
We also provide background on the one-dimensional bin-packing problem and submodularity. 

\subsection{Review on Graph Theory}
Let $G=(V,E,W)$ be a weighted undirected graph without loops and multiple edges, where $V$ is the set of verties, $E$ is the set of edges, and $W$ is the vertex weighting function such that $W:2^V\mapsto \mathbb{R}^+$. 
For any nonempty set $S\subseteq V$, $W(S) = \sum_{u \in S} W(u)$ is the weight of $S$. 

We use $V(G)$ and $E(G)$ to denote the set of vertices and edges in $G$, and use $e(u,v)$ to denote the edge that connects vertices $u,v\in V$. 
Let $G[V']$ be the subgraph of $G$ induced by $V'$, $\delta_G(v)$ the degree of vertex $v$, and $\Delta_G$ the maximum degree of $G$. 


\begin{mydef}[(Maximum) Independent Set (IS)]
Given a weighted undirected graph $G=(V,E,W)$, a subset $I \subseteq V$ is an \textit{independent set} of $G$ if for any two vertices $u,v \in I$, $e(u,v) \notin E$. 
An independent set $I$ of $G$ is \textit{maximum} if there is no independent set $I' \neq I$ of $G$ such that $W(I) < W(I')$.
\end{mydef}

The \textit{maximum weighted independent set} (MWIS) problem is to find the maximum independent set. 
When each vertex has an equal weight of $1$ (i.e., unweighted), it becomes the MIS (maximum independent set) problem.
As one of most important NP-hard problems \cite{halldorsson2000approximations}, there are no efficient algorithms in sight for MWIS, and heuristic methods (e.g., greedy strategies) are often used to obtain an approximate solution with certain performance guarantee. 
Denote the weight of a maximum IS of $G$ by $\theta(G)$, and the weight of the solution obtained by algorithm $A$ by $A(G)$.
The \textit{performance ratio} is defined by $\rho_A = \inf_G \frac{A(G)}{\theta(G)}$.

\begin{mydef}[(Maximal) Clique]
Given an undirected graph $G=(V,E)$, a subset $S\subseteq V$ is a clique of $G$, if for any two $u,v\in S$, $e(u,V)\in E$.
A clique is maximal if it cannot be extended by including one more adjacent vertex. 
\end{mydef}

\subsection{One-Dimensional Bin-Packing Problem}
The classic one-dimensional bin-packing problem \cite{coffman1978application,eilon1971loading,dosa2007tight, coffman1996approximation} is as follows: given $n$ items with sizes $s_1,s_2,...,s_n \in \mathbb{R}^+$, we want to find the smallest number of bins, each having a capacity of $C$, such that each item is packed into exactly one of the bins, and the sum of the sizes of the items in each bin is no more than $C$. 
It is well known that the bin-packing is NP-hard \cite{coffman1978application}, and algorithms based on heuristics such as the First Fit Decreasing algorithm \cite{eilon1971loading,dosa2007tight} are often used to find near-optimal solutions. 
A comprehensive survey on this topic is available in \cite{coffman1996approximation}.


\subsection{Submodularity}\label{sec:submodularity}
Submodularity is a property of set functions that captures the \textit{diminishing returns} behavior, that is, adding a new element introduces greater incremental benefits, if there are fewer elements so far, and less, if there are more elements.  
The formal definition is the following.

\begin{mydef}[Submodularity]
Given a finite set $V$, a function $f:2^V\mapsto \mathbb{R}$ is submodular if, for any subsets $S,T \subseteq V$, 
\begin{equation}
f(S) + f(T) \geq f(S\cap T) + f(S\cup T).
\end{equation}
$f$ is supermodular if $-f$ is submodular.
\end{mydef}

An equivalent definition is the following \cite{fujishige2005submodular}. 
A set function is submodular if, for any sets $S \subseteq T\subseteq V$ and any $v\in V\setminus T$, 
\begin{equation}
f(S \cup \{v\}) - f(S) \geq f(T \cup \{v\}) - f(T). \label{eq:equivalent_subomdular_def}
\end{equation}

Another useful property is \textit{monotonicity},  defined as follows. 

\begin{mydef}[Monotonicity]
Given a finite set $V$, a function $f: 2^V \mapsto \mathcal{R}$ is monotonic (or monotone) if, for any set $S\subseteq V$ and any $v\in V\setminus S$, $f(S \cup \{v\}) \geq f(S)$. 
\end{mydef}


If a set function $f(S)$ is submodular (and monotone), we can develop efficient algorithms for the following constrained optimization problems,
\begin{align}
\max\{f(S): S\in \mathcal{I}(\mathcal{M})\} \text{ and }\max\{f(S): S\in \mathcal{B}(\mathcal{M})\}.
\end{align}
where $\mathcal{I}(\mathcal{M})$ is the set of \textit{independent sets} and $\mathcal{B}(\mathcal{M}) \subseteq \mathcal{I}(\mathcal{M})$ is the set of bases of a \textit{matroid} $\mathcal{M}$, defined as follows.

\begin{mydef}[Matroid]
Let $V$ be a finite set, and let $\mathcal{I}$ be a collection of subsets of $V$. 
A set system $\mathcal{M}=(V, \mathcal{I})$ is a matroid if the following three conditions hold: (i) $\emptyset \in \mathcal{I}$, (ii) if $B \in \mathcal{I}$, then $A \in \mathcal{I}$ for all $A \subseteq B$, and (iii) if $A,B\in \mathcal{I}$ and $|A|<|B|$, then there exists $v \in B\setminus A$ such that $(A \cup \{v\}) \in \mathcal{I}$.
\end{mydef}

%The collection $\mathcal{I}$ is referred to as the set of \textit{independent sets} of the matroid $\mathcal{M}$. 
Each maximal independent set is a \textit{basis}. 
It can be shown that all bases of a matroid have the same size. 
The following lemma describes a property of submodular functions over matroid bases. 

\begin{mylemma}[\hspace{1sp}\cite{lee2010maximizing}]
Let $\mathcal{M}=(V,\mathcal{I})$ be a matroid, and let $f:2^V \mapsto \mathbb{R}$ be a submodular function defined on $V$. 
Let $S$ be a matroid basis such that, for all $u$ and $v$ with $u\in S$, $v\notin S$ and $(S \setminus \{u\} \cup \{v\}) \in \mathcal{I}$, $(1+\epsilon) f(S) \geq f(S \setminus \{u\} \cup \{v\})$. 
Then for any basic $C$ of $\mathcal{M}$, 
\begin{equation}
2(1+\epsilon) f(S) \geq f(S\cup C) + f(S \cap C).
\end{equation}
\end{mylemma}

The following lemma defines a sub-class of matroids called \textit{partition matroids}. 

\begin{mylemma}[Partition Matroid]\label{lemma:partition_matroid}
Let $V$ be a finite set, and $V_1$, ..., $V_m$ be a partition of $V$, that is, a collection of sets such that $V_1 \cup ... V_m=V$ and $V_i\cap V_j = \emptyset$ for $i\neq j$. 
Let $k_1$, ..., $k_m$ be a collection of nonnegative integers. 
Define a set $\mathcal{I}$ by $A \in \mathcal{I}$ iff $|A \cap V_i| \leq k_i$ for all $i=1,...,m$. 
Then $\mathcal{M}=(V, \mathcal{I})$ is a matroid, called a partition matroid. 
\end{mylemma}

